On the Resilience of Biometric Authentication Systems against Random Inputs

We assess the security of machine learning based biometric authentication systems against an attacker who submits uniform random inputs, either as feature vectors or raw inputs, in order to find an accepting sample of a target user. The average false positive rate (FPR) of the system, i.e., the rate at which an impostor is incorrectly accepted as the legitimate user, may be interpreted as a measure of the success probability of such an attack. However, we show that the success rate is often higher than the FPR. In particular, for one reconstructed biometric system with an average FPR of 0.03, the success rate was as high as 0.78. This has implications for the security of the system, as an attacker with only the knowledge of the length of the feature space can impersonate the user with less than 2 attempts on average. We provide detailed analysis of why the attack is successful, and validate our results using four different biometric modalities and four different machine learning classifiers. Finally, we propose mitigation techniques that render such attacks ineffective, with little to no effect on the accuracy of the system.

==> Acceptance Region_camera_ready/biometric.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Evaluation on Biometric Systems}
\label{sec:realscheme}

To evaluate the issue of acceptance region on real-world biometric systems, we chose four different modalities: gait, touch, face and voice. The last two modalities are used as examples of user authentication at the point of entry into a secured system, whilst gait and touch are often used in continuous authentication systems~\cite{barbello2016continuous}. We first describe the four biometric datasets, followed by our evaluation methodology, the machine learning algorithms used, and finally our results and observations.
%used process for creating, verifying and testing biometric user models, we will describe the four types of machine learning algorithms utilized for each modality, finally we display 
%\hassan{Why didn't we use fingerprint?}\ben{As fingerprint matching techniques are a well developed field that predates the use of machine learning, thus a majority of fingerprint systems leverage convectional distance based metrics to perform an authentication decision, as opposed to a machine learning solution.}

\subsection{The Biometric Datasets}
\label{sub:datasets}
%We strive to create realistic, yet reproducible biometric systems by curating publicly available datasets. Here we introduce our datasets of Gait, Touch, Face and Voice.

\subsubsection{Activity Type (Gait) Dataset}
The activity type dataset \cite{anguita2013public}, which we will refer to as the ``gait'' dataset, was collected for human activity recognition. Specifically its aim is to provide a dataset for determining if a user is sitting, laying down, walking, running, walking upstairs or downstairs, etc. However, as the dataset retains the unique identifiers for users per biometric record, we re-purpose the dataset for authentication. This dataset contains 30 users, with an average of $343 \pm 35$ ($\text{mean} \pm \text{SD}$) biometric samples per user, there is an equal number of activity type samples for each user. For the purpose of authentication, we do not isolate a specific type of activity. Instead, we include them as values of an additional feature. The activity type feature increases the total number of features to 562. We will refer to these features as \emph{engineered} features as they are manually defined (e.g., by an expert) as opposed to \emph{latent} features extracted from a pre-trained neural network for the face and voice datasets. 


%regarded as ``Engineered'' features as they are statistics computed from the timeseries contained in each biometric sample, without any additional abstraction. We make this distinction as the features within Face and Voice datasets are latent features extracted from a pre-trained neural network.
%The first step in utilizing this dataset is to unify the activity label with the respective samples, as our objective in authentication is not to label the activities, instead we treat the activity type as an additional feature, increasing the number of features to 562.

\subsubsection{Touch Dataset}
The UMDAA-02 Touch Dataset \cite{mahbub2016active} is a challenge dataset to provide data for researchers to perform baseline evaluations of new touch-based authentication systems. Data was collected from 35 users, with an average of $3667 \pm 3012$ 
%($mean \pm SD$)
swipes per user. This dataset was collected by lending mobile devices to the participants over a prolonged period of time. The uncontrolled nature of the collection produces a dataset that accurately reflects swipe interactions with constant and regular use of the device. This dataset contains every touch interaction performed by the user including taps. In a pre-processing step we only consider sequences with more than 5 data points as swipes. Additionally, we set four binary features to indicate the direction of the swipe, determined from the dominant vertical and horizontal displacement. We retained all other features in \cite{mahbub2016active} bar inter-stroke time, as we wished to treat each swipe independently, without chronological order. We substitute this feature with half-time of the stroke. This produces a total of 27 engineered touch features. 

\subsubsection{Face Dataset}
\label{subsub:face-dataset}
%Given the large number of face information databases available, we choose the CASIA dataset, as the pre-trained facenet model we use in the extraction of embeddings was originally trained on the VGGFace2 dataset \cite{cao2018vggface2}. 
FaceNet~\cite{schroff2015facenet} proposes a system based on neural networks that can effectively learn embeddings (feature vectors) that represent uniquely identifiable facial information from images. Unlike engineered features, these embeddings may not be directly explainable as they are automatically extracted by the underlying neural network. This neural network can be trained from any dataset containing labeled faces of individuals. There are many sources from which we can obtain face datasets, CASIA-WebFace~\cite{yi2014learning}, VGGFace2~\cite{cao2018vggface2} and Labeled Faces in the Wild (LFW)~\cite{LFWTechUpdate} are examples of such datasets. However, with a pre-trained model, we can conserve the time and resources required to re-train the network. The source code for FaceNet~\cite{facenet-source}
%\footnote{\url{https://github.com/davidsandberg/facenet}}
contains two pretrained models available for public use (at the time of writing): one trained on CASIA-WebFace, and another trained on VGGFace2. We opt to use a model pre-trained on VGGFace2\footnote{(20180402-114759) is the identifier of pre-trained model used.} 
%\hassan{<-- What are these numbers?}\ben{the exact pre-trained model used}
, while retaining CASIA-WebFace as our dataset for classifier training. We choose to use different datasets for the training of the embeddings and the classifiers to simulate the exposure of the model to never before seen data. Our face dataset is a subset of CASIA-WebFace containing only the top 100 identities with the largest number of face images (producing $447 \pm 103$ images per individual). This model produces 512 latent features from input images of pixel size 160x160 which have been centered and aligned. Recall that face alignment involves finding a bounding box on the face on an image, before cropping and resizing to the requested dimensions.


%The dataset we use is the CASIA-WebFace celebrity face dataset, from this dataset, we select 100 users with the largest number of images.
%We then configure Facenet to align and crop the face images, such that the image is of the same dimension (pixel size), and the celebrities face is centered and aligned within the image boundaries.
%Following the image pre-processing steps, we use the pre-trained Inception model (20180402-114759) that was trained on the VGGFace2 dataset, following the Inception ResNet v1 architecture. We use this pre-trained network to extract 512 latent features from our aligned facial images. Finally we normalize the latent features across the population of 100 users, between 0 and 1.

%\hassan{The following is not clear: we use CASIA dataset because facenet model uses VGGFace2 dataset? How are they related? And why mentioned LFW dataset?}
%We note that an alternative face dataset is Labelled Faces in the Wild (LFW) \cite{LFWTechUpdate, learned2016labeled}.

\subsubsection{Speaker Verification (Utterances)}% 
%\hassan{Needs a rewrite}\ben{rewritten}
VoxCeleb~\cite{nagrani2017voxceleb}, and VoxCeleb2~\cite{chung2018voxceleb2} are corpuses of spoken recordings by celebrities in online media. These recordings are text-independent, i.e., the phrase uttered by the user is not pre-determined. Text-independent speaker verification schemes depart from text-dependent verification schemes in which the individual is bound to repeat a pre-determined speech content. Thus, the task of text-independent verification (or identification) is to distinguish how the user speaks as an individual, instead of how the user utters a specific phrase. The former objective is an arguably harder task. Despite the increased difficulty, researchers have trained neural networks to convert speaker utterances into a set of latent features representing how individuals speak. These works have also released their models to the public, increasing the accessibility of speaker verification to developers. We opt to use the pre-trained model of VoxCeleb~\cite{nagrani2017voxceleb}, with utterances from VoxCeleb2~\cite{chung2018voxceleb2}. From VoxCeleb2, we only use the test portion of the dataset, which contains 118 Users with an average of $406 \pm 87$ utterances. VoxCeleb was trained as a Siamese neural network~\cite{siamese-bromley} for one-shot comparison between two audio samples. A Siamese network consists of two identical branches that produce two equal size outputs from two independent inputs for distance comparison. To fit the pre-trained model into our evaluation of ML-based models, we extract embeddings from one of the twin networks and disregard the second branch. The 1024-length embedding is then used as the feature vector within our evaluation.

\subsection{Evaluation Methodology}

% In this section we provide an overview of our attack. An attacker samples an input vector from $U(0,1)$, of length $n$, to be submitted to a user's trained model for authentication access. As the attacker assumes no other prior knowledge of the modality, each feature is treated as I.I.D. We also note that our vectors are sampled without replacement, to better simulate the attack conditions of an attacker starting fresh. We call the proportion of 1 million generated samples that have been incorrectly accepted as positive to be the Acceptance Region of the model, and hence a measure of the effectiveness of the attack.

% The remainder of the paper is laid out as follows, we will first reconstruct and demonstrate the attack on four biometric authentication schemes that have been recreated from publicly accessible datasets. These biometrics include Activity Gait, Facial recognition, Touch Behaviour, and Speech Utterances. Following this attack, we will demonstrate an attack on a synthetic dataset in which we control the parameters, allowing us to observe the relationship between the acceptance region and the training dataset. Finally we test a simple, but scalable mitigation strategy to minimize the acceptance region of the trained models.

\label{sub:eval-method}
%The procedure taken to evaluate the real biometric datasets is the same as the procedure on the synthetic dataset.
In our creation of biometric models for each user, we seek to obtain the baseline performance of the model with respect to the ability of negative user samples gaining access (i.e. FPR), and the measured Acceptance Region (AR). We use the following methodology to evaluate these metrics for each dataset and each classification algorithm.
\begin{enumerate}[leftmargin=5mm]
    \item We min-max normalize each extracted feature over the entire dataset between 0 and 1.
    %\hassan{Is this done after feature extraction or before feature extraction?} \ben{we normalize on the extracted features.}
    \item We partition the dataset into a $(70\%, 30\%)$ split for training and testing sets, respectively.
    \item For both training and testing samples, we further sample an equal number of negative samples from every other user such that the total number of negative samples are approximately equal to the number of samples from the target user, representing the positive class, i.e., the positive and negative classes are balanced.
    \item Using the balanced training set from step 3, we train a two-class classifier defining the target user set as the positive class, and all remaining users as negative.
    \item We test the trained model using the balanced testing set from step 3. This establishes the FRR and FPR of the system.
    \item We uniformly sample one million vectors from $\mathbb{I}_n$, where $n$ is the dimension of the extracted features. Testing the set of vectors against the model measures the acceptance region (AR).
    \item We record the confidence values of the test prediction for the user's positive test samples, other users' negative test samples, and the uniformly sampled vectors. These confidence values produce ROC curves for FRR, FPR and AR.
    \item Repeat steps 3-7 by iterating through every user in the dataset as the target user.
\end{enumerate}

\begin{remark}
\label{rem:monte-carlo}
%
In general, the decision regions (accept and reject in the case of authentication) learned by the classifiers can be quite complex~\cite{region-dnn}. Hence, it is difficult to determine them analytically, despite the availability of learned model parameters. We instead use a Monte Carlo method by sampling random feature vectors from $\mathbb{I}_n$ where each feature value is sampled uniformly at random from $\mathbb{I}$. With enough samples (one million used in our experiments, \blue{ and averaged over 50 repetitions}), the fraction of random samples accepted by the classifier serves as an estimate of the acceptance region as defined by Eq.~\ref{eq:ar} due to the law of large numbers.
\end{remark}

\blue{
\begin{remark}
Our evaluation of the biometric systems is using the mock attacker model (samples from the negative class modelled as belonging to an attacker) as it is commonly used~\cite{eberz2017evaluating}. We acknowledge that there are other attack models such as excluding the data of the attacker from the training set~\cite{eberz2017evaluating}. Having the attacker data included in the training dataset, as in the mock attacker model, yields better EER. On the other hand, it is also likely to lower the AR of the system, due to increased variance in the negative training dataset. Thus, the use of this model does not inflate our results.
\end{remark}
}

\blue{
\begin{remark}
\label{rem:balanced}
We have used balanced datasets in our experiments, i.e., the number of positive and negative samples being the same. It is true that a balanced dataset is not ideal for minimizing AR; more negative samples may reduce the acceptance region. However, an unbalanced dataset, e.g., more negative samples than positive samples, may be biased towards the negative class, resulting in misleadingly high accuracy~\cite{eberz2017evaluating, sugrim2019robust}. A balanced dataset yields the best EER without being biased towards the positive or negative class.
% We note that in this work we use balanced datasets as a means to overcome the scalability issues presented by using other users as a negative class. We used a balanced dataset (equal number of positive and negative samples) since it yields the best EER without being biased towards the positive or negative class, e.g., [1],  [reference 9 in the paper]. . But without the acknowledgement of AR issue, scheme designers may continue to opt for this best case scenario to report EER. 
\end{remark}
}

\subsection{Machine Learning Classifiers}
Our initial hypothesis (Section~\ref{sec:attack_def}) stipulates that AR is related to the training data distribution, and not necessarily to any weakness of the classifiers learning from the data. To demonstrate this distinction, we elected four different machine learning algorithms: Support Vector Machines (SVM) with a linear kernel (LinSVM), SVM with a radial basis function kernel (RBFSVM), Random Forests (RNDF) and Deep Neural Networks (DNN). Briefly, SVM uses the training data to construct a decision boundary that maximizes the distance between the closest points of different classes (known as support vectors). The shape of this boundary is dictated by the kernel used; we test both a linear and a radial kernel. 
%
Random Forests is an aggregation of multiple decision tree learners formally known as an ensemble method. Multiple learners in the aggregation are created through bagging, whereby the training dataset is split into multiple subsets, each subset training a distinct decision tree. The decisions from the multiple models are then aggregated to produce the random forest's final decision. 
%
DNNs are a class of machine learning models that contain hidden layers between an input and an output layer; each layer containing neurons that activate as a function of previous layers. Specifically we implement a convolutional neural network with hidden layers leading to a final layer of our two classes, accept and reject.
%
All four of these machine learning models are trained as supervised learners. As such, we provide the ground truth labels to the model during training. 
%this is in contrast to unsupervised learners which attempt to create their own class groupings from unlabelled data.

%\paragraph{Machine Learning Classifier Parameters}
The linear SVM was trained with $C=10^4$, and default values included within Scikit-learn's Python library for the remaining parameters \cite{scikit-learn}. For radial SVM we also used $C=10^4$ while keeping the remaining parameters as default. The Random Forests classifier was configured with 100 estimators. DNNs were trained with TensorFlow Estimators~\cite{tensorflow-estimators}
%\footnote{\url{https://www.tensorflow.org/guide/estimators}}
with a varying number of internal layers depending on the dataset. The exact configurations are noted in Appendix~\ref{sec:dnn_config}.

\begin{remark}
%\hassan{Requires rewrite}\ben{partial}
We reiterate that our trained models are reconstructions of past works.
%We emphasize that we are not directly attacking trained models produced by previous authentication work,
%as the majority of them contain user data that is not publicly released for privacy and ethical reasons. 
%Additionally, our re-evaluation of different machine learning algorithms changes the implementation of previously proposed schemes. 
However, we endeavor that our models recreate error rates similar to the originally reported values on the same dataset. On Mahbub et al.'s touch dataset~\cite{mahbub2016active}, the authors achieved 0.22 EER with a RNDF classifier, by averaging 16 swipes for a single authentication session. We are able to achieve a comparable EER of 0.21 on RNDF without averaging. 
%The EERs on the other 3 classifiers are higher but we maintain these as they are trained on the same dataset. 
For face authentication, we evaluate a subset of CASIA-Webface, consequently there is no direct comparison. The original Facenet accuracy in verifying pairs of LFW~\cite{LFWTechUpdate} faces is 98.87\%~\cite{schroff2015facenet}, but our adoption of model-based authentication is closer to~\cite{explainable-AI}, unfortunately the authors have fixed a threshold for 0 FPR without reporting their TPR.
Nagrani, Chung and Zisserman's voice authenticator~\cite{nagrani2017voxceleb} reports an EER of 0.078 on a neural network. Our classifiers achieve EERs of 0.03, 0.02, 0.04 and 0.12, which are within range of this benchmark. Our gait authenticator is the exception, it has not been evaluated for authentication with it's mixture of activity types. However, a review of gait authentication schemes can be found at~\cite{sprager2015inertial}.
%Thus, we believe our evaluation is representative of results on real-world schemes for these modalities. 

%\hassan{[REF: which dataset reproduces which reported ERR]}\ben{quote ml-leak format, faces(Hu\_Discriminative\_Deep\_Metric\_2014\_CVPR\_paper.)}.

%\hassan{We have to mention which ones are closely recreated with references} \ben{All of them}
\end{remark}

\subsection{Acceptance Region: Feature Vector API}
%\hassan{A lot of the info here should go into when we are describing these datasets at the beginning of this section.}

%\hassan{I think for each of these datasets and classifiers, we should also highlight cases of individual target users where AR was exceptionally high yet FPR and TPR were good. Otherwise it gives an impression that AR is in most cases close to FPR. Note that these are average readings. For some users, we would have AR less than FPR and for others we won't. I think it is important to highlight this here to make our results stand out}\ben{in progress}

%\ben{one point we highlight is this effect is both model agnostic, and biometric modality agnostic. It may help reiterate our point if we do not separate the results discussion between the modalities (we would also be saying nearly the same conclusion for each modality.)}

In this section, we evaluate the acceptance region (AR) by comparing it against FPR for all 16 authentication configurations (four datasets and four classifiers). In particular, we display ROC curves showing the trade-off between FPR and FRR against the acceptance region (AR) curve as the model thresholds are varied. These results are averaged over all users. While this gives an average picture of the disparity between AR and FPR, it does not highlight that for some users AR may be substantially higher than FPR, and vice versa. In such a case, the average AR might be misleading. Thus, we also show scattered plots showing per-user AR and FPR, where the FPR is evaluated at EER. The per-user results have been averaged over 50 repetitions to remove any bias resulting from the sampled/generated vectors. The individual user AR versus FPR scatter plots are shown in Figure~\ref{fig:all_ind}, and the (average) AR curves against the ROC curves are shown in Figure~\ref{fig:all_roc}. 

%In this subsection, we will display 
%(Note that the displayed metric is FRR, the False Rejection Rate, and is equal to FRR = 1 - TPR). 
%These are average ROC curves (with FPR and AR) across all users will be shown in the following section. We will also be noting the EER of FRR and FPR, and the resulting AR if the confidence threshold was set based on this EER. 
%
%One additional stipulation was that it was difficult to predict the AR of a user (and hence security of the system) based on the FPR alone, for this we display a scatter plot with points corresponding to a user model's FPR and AR.

\begin{remark}
EER is computed in a best effort manner, with only 100 discretized threshold values, to mitigate the storage demands of the 1M uniformly random vectors measuring AR. Unfortunately, there are some instances whereby the FRR and FPR do not match exactly, as the threshold step induces a large change in both FRR and FPR. Only 1/16 classifiers exhibit an FPR-FRR discrepancy greater than 1\%.
\end{remark}


%In many of the results the AR will be observed close to the FPR, But we note that the AR is accessible by the attacker with near-zero knowledge of the system. A random attack requires at the very least knowing what the authentication system records. We also provide in Figure~\ref{fig:individual_ar-fpr} the relationship between the AR and FPR of every user within their respective datasets. These results aim to display that users with seemingly adequate FPR performance, may still be susceptible to a large AR.

\begin{figure}[t]
    \centering
  \subfloat[Gait\label{fig:gait_ind}]{%
       \includegraphics[width=0.46\linewidth]{images/gait_proba_ind-crop.pdf}}
    \hfill
  \subfloat[Touch\label{fig:touch_ind}]{%
        \includegraphics[width=0.46\linewidth]{images/touch_proba_ind-crop.pdf}}
    \vspace{-0.3cm}
    \\
  \subfloat[Face\label{fig:face_ind}]{%
        \includegraphics[width=0.46\linewidth]{images/face_proba_ind-crop.pdf}}
    \hfill
  \subfloat[Voice\label{fig:voice_ind}]{%
        \includegraphics[width=0.46\linewidth]{images/voice_proba_ind-crop.pdf}}
  \vspace{-0.2cm}
  \\
  \caption{Individual user scatter of AR and FPR. In a majority of configurations, there is no clear relationship between AR and FPR, with the exception of the RBFSVM and DNN classifiers for face and voice authentication. 
  %Two modalities that have good authentication performance.}
  \vspace{-1mm}
  }
  
  \label{fig:all_ind} 
\end{figure}



\begin{figure*}
  \centering
  \subfloat[Gait Average ROC\label{fig:gait_roc}]{%
       \includegraphics[width=1.0\linewidth]{images/gait_proba_roc-crop.pdf}}\\
  \subfloat[Touch Average ROC\label{fig:touch_roc}]{%
        \includegraphics[width=1.0\linewidth]{images/touch_proba_rand_roc-crop.pdf}}\\
  \subfloat[Face Average ROC\label{fig:face_roc}]{%
        \includegraphics[width=1.0\linewidth]{images/face_proba_rand_roc-crop.pdf}}\\
  \subfloat[Voice Average ROC\label{fig:voice_roc}]{%
        \includegraphics[width=1.0\linewidth]{images/voice_proba_roc-crop.pdf}}
  \caption{ROC curve versus the AR and RAR curves for all configurations. The EER is shown as a dotted vertical blue line. The FRR, FPR, AR and RAR values shown in the legend are evaluated at EER (FPR = FRR). The RAR is only evaluated on the Touch and Face datasets.} %The two modalities with the lowest EER is Face and Voice are the modalities that had features extracted from a pre-trained neural network. Both these networks do not observer the AR behaviour deviating too far from the FPR, with the exception of the RNDF classifier. The RNDF classifier observes a rapid rise in the success of the random attack, well above the FPR if the threshold were to be lowered. For Face, without any change in threshold it is already susceptible to this random attack.}
  %\hassan{It will be helpful to draw the line here where EER equals RAR (since the two axis are not of the same length)}
  \label{fig:all_roc} 
\end{figure*}


\subsubsection{Gait Authentication}
\label{sec:classify_gait}
%The Activity Type Dataset \cite{anguita2013public} is a dataset that was collected for the expressed purpose of identifying the type of activity a human user is carrying out.
%Specifically it aimed to provide a dataset for determining if a user is sitting, laying down, walking, running, walking upstairs, walking downstairs.
%
%Their dataset contains 30 users, with approximately 300 training samples per user across all activity types. We note this dataset provides already extracted features previously utilized for activity recognition, we re-purpose these features with no modification for user verification (authentication).
%
%The first step in utilizing this dataset is to unify the activity label with the respective samples, as our objective in authentication is not to label the activities, instead we treat the activity type as an additional feature, increasing the number of features to 562.
%
%\paragraph*{Results}
Figure~\ref{fig:gait_ind} shows AR against FPR of every user in the activity type (gait) dataset. Recall that in this figure FPR is evaluated at EER. The dotted straight line is the line where AR equals FPR (or ERR). We note that there is a significant proportion of users for which AR is greater than FPR, even when the latter is reasonably low. For instance, in some cases AR is close to 1.0 when the FPR is around 0.2. Thus, a random input attack on systems trained for these target users will be successful at a rate significantly higher than what is suggested by FPR. We also note that the two SVM classifiers have higher instances of users for whom AR surpasses FPR. Figure~\ref{fig:gait_roc} shows the AR curve averaged across all users against the FPR and FRR curves for all four classifiers. We can see that AR is higher than the ERR (represented by the dotted vertical line) for the two SVM classifiers. For the remaining two classifiers, AR is lower than EER. However, by looking at the AR curve for RNDF, we see that the AR curve is well above the FPR curve when $\text{FRR} \le 0.3$. This can be specially problematic if the threshold is set so as to minimize false rejection at the expense of false positives. We also note that the AR curve for DNN closely follows the FPR curve, which may suggest that the AR is not as problematic for this classifier. However, by looking at Figure~\ref{fig:gait_ind}, we see that this is misleading since for some users the AR is significantly higher than FPR, making them vulnerable to random input attacks. Also, note that the AR generally decreases as the threshold is changed at the expense of FRR. However, except for RNDF, the AR for the other three classifiers is significantly higher than zero even for FRR values close to 1.

% same as EER  for this figure  we can see that there is not a strong correlation between the acceptance region and the typically reported FPR-EER.
% On the other hand when focusing on system averages, irrespective of the specific user, we observe from Figure~\ref{fig:gait_roc} that in both instances of SVM the average AR is larger than the equivalent EER. Unlike RNDF and DNN, were we observe an AR similar to the EER. 

% \begin{figure*}[th!]
% 	\centering
%     \includegraphics[width=1.0\textwidth]{images/gait_proba_roc-crop.pdf}
%     \vspace{-0.5cm}
%   	\caption{Gait authentication results, the EER is marked on the diagrams.}
%  	\label{fig:gait_roc}
% \end{figure*}

% \begin{figure}[th!]
% 	\centering
%     \includegraphics[width=1.0\linewidth]{images/gait_proba_ind.pdf}
%     \vspace{-0.5cm}
%   	\caption{Scatter of FPR-EER and the corresponding AR of Gait models, each point represents one user. \ben{will place all 4 diagrams into the same main figure.} \ben{needs B/W friendliness}}
%  	\label{fig:gait_ind}
% \end{figure}

% \begin{figure}[ht] 
%   \label{fig7} 
%   \begin{minipage}[b]{0.5\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{images/gait_proba_ind-crop.pdf} 
%     \vspace{-0.5cm}
%     \caption{Gait}\label{fig:gait_ind}
%     \vspace{4ex}
%   \end{minipage}%%
%   \begin{minipage}[b]{0.5\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{images/touch_proba_ind-crop.pdf} 
%     \vspace{-0.5cm}
%     \caption{Touch}\label{fig:touch_ind}
%     \vspace{4ex}
%   \end{minipage} 
%   \begin{minipage}[b]{0.5\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{images/face_proba_ind-crop.pdf} 
%     \vspace{-0.5cm}
%     \caption{Face}\label{fig:face_ind}
%     \vspace{4ex}
%   \end{minipage}%% 
%   \begin{minipage}[b]{0.5\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{images/voice_proba_ind-crop.pdf} 
%     \vspace{-0.5cm}
%     \caption{Voice}\label{fig:voice_ind}
%     \vspace{4ex}
%   \end{minipage}
%   \caption{Individual user scatter of AR and FPR}
% \end{figure}



% \subsection{Up Swipes dataset}
% \label{sec:swipes}
% \ben{Potential cut, as this dataset is not publicly accessible/ethics consideration.}

% A Swipes classifier is constructed from a dataset of swipes in the upwards direction, 45 Users with $\ge20$ swipes had biometric models constructed for them.

% The Machine learning models were trained with a 20/80 \% random split of the entire dataset, and repeated for validation.

% We use a ensemble approach for the machine learning models, as we adopt a two-class classification problem trained on both the user's own positive data, and other users as negative data. To address training imbalance, we evenly sample from all other users to create a set of negative samples approximately equal to the user's positive training samples. Due to the randomness of sampling, we generate 20 versions of ML model with different sampling of the negative class. The final ensemble decision is made by majority vote.

% \subsubsection{Why do some users have a high Acceptance Region}
% In order to predict why some users are subject to larger acceptance regions, we focused on the random forest classifier, as it is able to provide a relative importance of features post-training. We normalize the standard deviation of the user's feature samples with this value of importance and observe a strong spear-man correlation between this metric and the acceptance region. This relationship indicates a vulnerability where features with a high standard deviation have been considered important for authentication. The larger distribution thus leaves a larger attack surface for randomly chosen values to successfully fall within valid bounds.

% \hassan{Is this the only reason? How about the negative class variation?}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\section{Real biometrics scheme}
%\label{sec:realscheme}


%\subsection{A Secure Mobile Authentication Alternative to Biometrics}
%\red{Will not work, due to protection offered by random projections}
%We test our idea on Azimpourkivi's ai.lock \cite{azimpourkivi2017secure}. We redeploy the code as provided in their paper, training only on the nexus image dataset (features have been pre-extracted from the Inception deep learning model). We then modify their test script to receive noise as the input vector, instead of an image's feature vector. Upon rerunning their system and with their optimized threshold, we obtain performance results of: TPR, FPR, FNR, TNR. After testing random attacks against all users, we obtain a Acceptance region of XXXX. The way we generate the noise is by creating a binary vector of equal length to the system input, and randomly populating it with 0s and 1s.



\subsubsection{Touch (Swipe) Authentication}
\label{sec:classify_touch}

%The touch based Authenticator.

%The paper originally releasing the dataset to the public provided a fixed set of features for their original evaluation. We re-implemented the feature extraction function of their features, bar Inter-stroke time, as we wished to treat each swipe independently. Instead substituting the feature with the half-time of the stroke. With the re-implemented system, we extracted features from the raw swipes, and performed our evaluation methodology.

% On only the features tagged with the 2 direction, we obtain the ROC curve seen in Figure \ref{fig:touch_roc}

%\paragraph*{Results}
% This touch authenticator objectively performs the worst of all four biometric modalities, largely due to the uncontrolled nature of collection, and the limited size of the feature-set extracted.
% Jumping ahead, the touch modality does not performing as well as the Face or Voice modality, however it is performing on par with the reported performance in the original paper releasing the dataset \cite{mahbub2016active}. Likely due to the limited set (27) of features used for evaluation. Nonetheless, this allows us to observe the AR when the model performance is not optimal. Given this performance, we observe that in both SVM classifiers the relative difference between the AR and FPR is larger than previously observed in gait, unlike the relatively minor variations in RNDF and DNN.

% Upon viewing the scatter of user AR and FPR, we observe an even weaker relationship between AR and FPR, in comparison to gait.

%\hassan{Are these averaged over multiple samples?} \ben{50 repetitions for each user, different data splits each time. Average ROC is averaged over all 50 and all users.}\hassan{No, I mean see footnote 2}\ben{we do not treat it in the continuous case, one sample is one sample, no averaging between samples} \hassan{Okay, this is probably the main reason behind high EER for both gait and touch}\ben{possibly}
The touch authenticator has the highest EER of all four biometric modalities. Very few users attained an EER lower than 0.2 as seen in Figure~\ref{fig:touch_ind}. This is mainly because we consider the setting where the classification decision is being made after each input sample. Previous work has shown EER to improve if the decision is made on an average vector of a few samples some work~\cite{unobservable, touchalytics, chauhan2017behaviocog}. Nevertheless, since our focus is on AR, we stick to the per-sample decision setting. Figure~\ref{fig:touch_ind} shows that more than half of the users have ARs larger than FPR, and in some cases where the FPR is fairly low (say 0.2), the AR is higher than 0.5. Unlike gait authentication where RNDF classifier had ARs less than FPR for the majority of the users, all four algorithms for touch authentication display high vulnerability to the AR based random input attack. When viewing average results in Figure~\ref{fig:touch_roc}, we observe the average AR curve to be very `flat' for both SVM classifiers and DNN. This indicates that AR for these classifier remains mostly unchanged even if the threshold is moved closer to the extremes. RNDF once again is the exception, with the AR curve approaching 0 as the threshold is increased.
%, the AR curve drops below the FPR curve and will no longer be overstated.


%Despite the large EER, like in the Gait models even larger ARs were observed, with more than half the users with ARs larger than FPR; however unlike Gait, where the RNDF classifier was able to resist the random attack, all ML algorithms for Touch displayed a high vulnerability. We suspect the poor EER is largely due to the uncontrolled nature of collection, and the limited feature-set extracted (27 features). Whilst it has been shown that averaging features between successive samples be improve the performance of continuous authentication \cite{chauhan2016gesture}, we do not employ such a strategy.




% \begin{figure*}[th!]
% 	\centering
%     \includegraphics[width=1.0\textwidth]{images/touch_proba_roc-crop.pdf}
%   	\caption{Touch authentication results, the EER is marked on the diagrams. \hassan{Why are we reporting AR seemingly where it intersects with the FRR curve rather than the AR that corresponds to the ERR mark as defined by FPR = FRR?} \ben{This is a good point, as we wanted to emphasize that a configuration currently chosen based on FPR may not offer sufficient AR protection.}}
%  	\label{fig:touch_roc}
% \end{figure*}

% \begin{figure*}[bth!]
% 	\centering
%     \includegraphics[width=1.0\textwidth]{images/touch_proba_rand_roc-crop.pdf}
%     \vspace{-0.5cm}
%   	\caption{Touch authentication results, the EER is marked on the diagrams. With RAR (Raw Acceptance Region) and AR (Acceptance Region).}
%  	\label{fig:touch_roc}
% \end{figure*}



\subsubsection{Face Authentication}
\label{sec:classify_face}
% We evaluate the acceptance region on the CASIA-WebFace\cite{yi2014learning} dataset, processed by Facenet \cite{schroff2015facenet}, a state of the art neural network trained on a large corpus of human faces to extract latent features from face images.
%The extracted latent features will be close between different face images of the same user, while far for different users.
%A common use case of Facenet is to perform Facial identification, However the n-class classification problem of identification can be adapted for authentication by redefining it as a binary classification problem. With a positive class as the returning user, and a negative class as not the returning user.
%
% \ben{
% We believe our reconstruction of the Facial recognition is sufficiently similar to real world facial authentication schemes, as it draws parallels to pending patent US15/864,232. Additionally there are API services dedicated to hosting different components of the facial recognition pipeline. Clarifai, for example hosts models dedicated to the extraction of \href{https://clarifai.com/models/face-embedding-image-recognition-model-d02b4508df58432fbb84e800597b8959}{face embeddings} within an uploaded image. A developer could then use any number of Machine Learning as a Service (MLaaS) providers to perform the final authentication step, without needing to pay the premium associated with a end-to-end facial recognition product.
% }

%The dataset we use is the CASIA-WebFace celebrity face dataset, from this dataset, we select 100 users with the largest number of images.
%We then configure Facenet to align and crop the face images, such that the image is of the same dimension (pixel size), and the celebrities face is centered and aligned within the image boundaries.
%Following the image pre-processing steps, we use the pre-trained Inception model (20180402-114759) that was trained on the VGGFace2 dataset, following the Inception ResNet v1 architecture. We use this pre-trained network to extract 512 latent features from our aligned facial images. Finally we normalize the latent features across the population of 100 users, between 0 and 1.

%The features discussed within the remainder of this section refers to the 512 extracted latent features.

% Table has been depreciated for ROC curves
% \begin{table}[ht!]
%     \centering
%     \begin{tabular}{|c|lll|}
%     \hline
%     & TPR & FPR & AR\\ \hline
%         Linear SVM & 0.9508 & 0.0528 & 0.1563\\
%         Radial SVM & 0.9586 & 0.0405 & 0.0089\\
%         Random Forests & 0.9214 & 0.0133 & 0.1919\\
%         Deep Neural Network &  0.8849 & 0.0274 & 0.0310\\
%         \hline
%     \end{tabular}
%     \caption{Facial authentication results \ben{We could plot ROC curves here, showing TPR, FPR and AR changes with threshold. Need to figure out how to vary threshold for DNN} \red{*Facenet NN ran for extraction, but DNN classifier not yet run.}
%     \red{**060219 - Tweaking hidden layers as current layer config is bad.}
%     \red{**070219 - Current config acceptable, but continuing to tweak}}
%     \label{tab:face_results}
% \end{table}
%\paragraph*{Results}
Figure~\ref{fig:face_ind} shows that AR is either lower or comparable to FPR for RBFSVM and DNN. Thus, the FPR serves as a good measure of AR in these systems. However, AR for most users is significantly higher than FPR for LinSVM and RNDF. This is true even though the EER of these systems is comparable to the other two as seen in Figure~\ref{fig:face_roc}. For LINSVM, we have an average AR of 0.15 compared to an EER of 0.05. For RNDF, the situation is worse with the AR reaching 0.78 against an EER of 0.03. We also note that while the AR is equal to FPR for DNN, its value of 0.10 is still worrisome to be resistant to random input attack. The relatively high FPR for DNN as compared to RBFSVM is likely due to a limited set of training data available in training the neural network.

%At first glance Figure~\ref{fig:face_ind} displays a distinct correlation between the AR and the FPR of a user's model. However this linear relationship is only substantial for the RBFSVM and DNN authenticatiors. Additionally, we observe that for both these RBFSVM and DNN the user ARs are consistently less than the EER. Thus in both the RBFSVM and DNN classifiers, the quoted security of the model in the form of EER has not been overstated, and even serves as an indicator for the AR behaviour of each user. On the other hand the LINSVM classifier, whilst consistent in EER, the AR of the user models varies substantially, not to mention the large AR for the relatively small FPR in both LINSVM (EER $\le 0.1$) and RNDF ((EER $\le 0.12$)).

%From the average ROC plots in Figure~\ref{fig:face_roc}, It is clear the facial recognition classifier performs better than the previous biometric modalities. We suspect that one primary reason for the discrepancy in performance, is the feature extraction process. Both gait and touch, consists of engineered statistical features derived from the raw timeseries, unlike the latent features that are extracted from a neural network trained on extremely large datasets for face and voice authentication. %\hassan{So, the use of DNN for gait and touch does not use latent features?} \ben{no, the DNN is just for the final binary classification task} \ben{When I say latent, I mean hidden/abstracted, statistical features e.g. mean, std, percentile would not be considered latent features.}. 
%We note that Linear SVM, Radial SVM and Random Forests exhibit near identical FPRs, however the resulting AR varies, the AR in the Radial SVM is lower than FPR, but for Linear SVM, and Random Forests, have ARs larger than FPR. The DNN implementation of the face authenticator reflects the same difference in FPR and AR as Radial SVM, but observes a worse performing FPR, likely due to a limited set of training data available in training the neural network.


% \begin{figure*}[th!]
% 	\centering
%     \includegraphics[width=1.0\textwidth]{images/face_proba_roc-crop.pdf}
%   	\caption{Face authentication results, the EER is marked on the diagrams.}
%  	\label{fig:face_roc}
% \end{figure*}


% \begin{figure*}[th!]
% 	\centering
%     \includegraphics[width=1.0\textwidth]{images/face_proba_rand_roc-crop.pdf}
%     \vspace{-0.5cm}
%   	\caption{Face authentication results, the EER is marked on the diagrams. With RAR (Raw Acceptance Region) and AR (Acceptance Region).}
%  	\label{fig:face_roc}
% \end{figure*}


\subsubsection{Voice Authentication}
\label{sec:classify_speech}
% We evaluate a large dataset of audio samples from celebrities who have been filmed and uploaded to YouTube \cite{nagrani2017voxceleb}\cite{chung2018voxceleb2}.
%The work as carried out by Nagrani et al. yields a large dataset of audio samples from celebrities who have been filmed and uploaded to YouTube \cite{nagrani2017voxceleb}. 
%To begin speaker verification is the process to verify that an audio sample has been spoken by a target user. Audio segments are considered utterances if there is no fixed phrase the speaker has to reproduce. Their work was later extended by Chung et al. that has yielded an even larger dataset \cite{chung2018voxceleb2}.
%Our test leverages the pre-trained model from the original VoxCeleb1 dataset, to ensure our model does not overfit the initial training data, we use the dataset of VoxCeleb2 on a pre-trained neural network model trained on VoxCeleb1.
%
%VoxCeleb1 was trained as a Siamese network for a one shot comparison between two audio samples. A Siamese network is two identical branches that produce two equal size outputs from two independent inputs. The similarity of these outputs are then compared for a distance metric which is checked against a pre-determined threshold to determine if these samples originate from the same user. To fit the VoxCeleb dataset into our existing evaluation pipeline, we take a similar approach to FaceNet, whereby embeddings from one of the twin networks are extracted and used as a representation of the original audio input. These embeddings are then used as the feature vectors within our machine learning algorithms.
%We focus on the test dataset of VoxCeleb2, as it contains 118 user with audios samples in the range of 500 to the 10s. As such we consider the 100 users with the most samples for this evaluation. 
%The Siamese network produces features of length 1024.

%\paragraph*{Results}
%Given the low FPR obtained from this modality across all classifier types, the difference between the FPR and the AR is also low. 
Figure~\ref{fig:voice_ind} shows that once again LinSVM and RNDF have a significant proportion of users with AR higher than FPR, whereas for both RBFSVM and DNN the AR of users is comparable to FPR. Looking at the average ARs in Figure~\ref{fig:voice_roc}, we see that interestingly RNDF exhibits an average AR of 0.01 well below the ERR of 0.04. The average suppresses the fact that there is one user in the system with an AR close to 1.0 even with an EER of approximately 0.1, and two other users with an AR of 0.5 and 0.3 for which the EER is significantly below 0.1. Thus these specific users are more susceptible to the random input attack. Only LinSVM has an average AR (0.08) higher than EER (0.03). The average AR of DNN is lower than EER (0.11), but it is still significantly high (0.08). For RBFSVM we have an average AR close to 0.  

% Individually in Figure~\ref{fig:voice_ind}, there are 3 user models with the RNDF classifier that are clearly visible outside the main cluster of users. One of these exceptions has an AR close to one with a seemingly benign EER of about 0.1 (albeit high relative to the other RBFSVM models), with the other two at 0.5 and 0.3 AR for an EER $< 0.5$. These specific users would be susceptible to the random attack, and the model would offer little to no security for them. Compounding the issue, from an average point of view in Figure~\ref{fig:voice_roc}, the AR for the RNDF classifier is 0.01, providing no indication for these outlying users of the vulnerability affecting only their models. In the remaining 3 classifiers the shape of the AR curves in Figure~\ref{fig:voice_roc} again mirrors the shape of the FPR curve, with RBFSVM and DNN having AR curves below FPR (-0.02 and -0.04 respectively), and LINSVM slightly above (+0.06) at the EER point and across the thresholds.

% \begin{figure*}[th!]
% 	\centering
%     \includegraphics[width=1.0\textwidth]{images/voice_proba_roc-crop.pdf}
%     \vspace{-0.5cm}
%   	\caption{Voice authentication results, the EER is marked on the diagrams.}
%  	\label{fig:voice_roc}
% \end{figure*}

\subsection*{Observations}
In almost every configuration, we can observe that the average AR is either higher than the FPR or at best comparable to it. Furthermore, for some users the AR is higher than FPR even though the average over all users may not reflect this trend. This demonstrates that an attacker with no prior knowledge of the system can launch an attack against it via the feature vector API. Moreover, for both the linear and radial SVM kernels, and some instances of the DNN classifier, we observe a relatively flat AR curve as the threshold is varied, unlike the gradual convergence to 1 experienced by the FPR and FRR curves. 
%This indicates that a large proportion of the feature space probed by the uniformly generated samples does not belong to the true positive region (See Section~\ref{sec:attack_def}), 
%and thus unaffected by minor changes in the decision threshold. The implication of 
%These classifiers that exhibit this flat response is they will 
These classifiers thus have a substantial acceptance region that accept samples as positives irrespective of the threshold. Random Forests is the only classifier where the AR curve shows significant drop as the threshold is varied. 
%\hassan{Still not clear. May be give a reference?} It is suspected that the ensemble nature of the classifier assists providing a large change in the AR. In the process of bagging the training data will provide each tree with a different subset of data. With multiple subsets of data the overall random forests ensemble it is more likely that a proportion of trees will exclude the unchanging acceptance regions (proximity to negative samples), in contrast to the SVM classifiers, whereby the region is either accepted or rejected given the single instance of data.
Random forests sub-divide the training dataset in a process called bagging, where each sub-division is used to train one tree within the forest. With different subsets of data, different training data points will be closer to different empty regions in feature space, thus producing varied predictions. Because the prediction confidence of RNDF is computed from the proportion of trees agreeing with a prediction, the lack of consensus within the ensemble of trees for the empty space may be the reason for the non-flat AR curve.

%In regards to the user-specific correlation between the Acceptance Region and the FPR, whilst not immediately obvious, we do observe a trend for the DNN classifier between the modalities, whereby systems with an overall lower FPR will tend to have a stronger relationship between AR and FPR. This also applies to a lesser extent for Radial SVM, but the same cannot be said for Linear SVM and Random Forests.

\subsection{Acceptance Rate: Raw Input API}
\label{sub:rar-results}
%Faux Raw Feature Input, Raw-AR (RAR)}

%\ben{extra section here to highlight the RAW results of Touch and Face.}
%In the previous section we evaluated the effectiveness of an attacker with minimal prior knowledge of the system with API access. However in the event that the attacker does not have API access, and only Raw Input access to the model, the attacker should still not posses a substantial chance of entry. 
The results from the feature vector API are not necessarily reflective of the success rate of a random input attack via the raw input API. One reason for this is that the feature vectors extracted from raw inputs may or may not span the entire feature space, and as a consequence the entire acceptance region. For this reason, we use the term \emph{raw acceptance rate} (RAR) to evaluate the probability of successfully finding an accepting sample via raw random inputs. To evaluate RAR, we select the touch and face biometric datasets. The raw input of the touch authenticator is a time-series, whereas for the face authentication system it is an image. 

% Thus, we evaluate the acceptance region for raw inputs. For this reason we evaluate the possibility of attacker access when raw inputs are generated. We select Touch and Face biometrics for this evaluation as the raw inputs take the form of a timeseries and a image respectively.

% By sampling uniform vectors from the feature space we have shown that an attacker is able to gain access at a sufficient rate with little to no cost. A more realistic attack scenario is if an attacker only has access to the system before the feature extraction process. As such we test the capability of an attacker with minimal knowledge of the biometric process in generating the raw inputs.

% A minimal amount of knowledge for an attacker in a facial authentication system is knowing only the size of the image, disclosed (and enforced) if the feature extraction process only accepts inputs of a fixed size. With this information, the attacker with no other knowledge and assumptions can effectively generate noise.

%\paragraph*{Raw Touch Input Results}
\subsubsection{Raw Touch Inputs}
%\footnote{\href{https://bitbucket.csiro.au/users/zha197/repos/touch-auth/browse/proba_rand/random_touch_features.py}{touch\_generation\_script\_here}} 
We used a continuous auto-regressive process (CAR)~\cite{timesynth-source}
%\footnote{\url{https://github.com/TimeSynth/TimeSynth}} 
to generate random timeseries. We opted for CAR due to the extremely high likelihood of time-series values having a dependence on previous values. This time-series was then min-max scaled to approximate sensor bounds. For example the \texttt{x}-position has a maximum and minimum value of 1980 and 0 respectively, as dictated by the number of pixels on a smartphone screen. Both the duration and  length of the time-series were randomly sampled from reasonable bounds: 0.5 to 2.0 seconds and 30 to 200 data-points, respectively. The time-series was subsequently parsed by the same feature extraction process as a legitimate time-series, and the outputs scaled on a feature min-max scale previously fit on real user data. In total we generate 100,000 time-series\blue{, which are used to measure RAR over 50 repetitions of the experiment.}


The results of our experiments are shown in  Figure~\ref{fig:touch_roc}, with the curve labeled RAR showing the raw acceptance rate as the threshold of each of the classifiers is changed. As we can see, the RAR is large and comparable to AR. This seems to indicate that the region spanned by random inputs covers the acceptance region. However, on closer examination, this happens to be false. The average volume covered by the true positive region for the touch dataset (cf. Section~\ref{sec:attack_def}) is less than $1.289 \times 10^{-4} \pm 5.462 \times 10^{-4}$, yet the volume occupied by the feature vectors extracted from raw inputs is less than $2.609 \times 10^{-6}$. This is significantly smaller than the AR for all four classifiers. We will return to this observation shortly.  


%This result contradicts held reservations about the feature extraction process restricting the possible feature space attainable by random raw samples.

%We compute the rectangular space of the users within the touch dataset. These users have an average $0.0001289 \pm 0.0005462$ ($mean \pm SD$), but the volume occupied by the raw inputs only covers $2.609 \cdot 10^{-6}$.

\subsubsection{Raw Face Inputs}
%Whilst an attack surface after the feature extraction module is realistic, it is desirable to consider how difficult it is to launch this attack from the raw image input. We test the hypothesis that given noise as the input to the feature extraction process, the output should also contain noisy features. And it is possible that the feature output is sufficiently noisy to interact with the acceptance region as we have seen with our uniform random input.

We generated 100,000 images of size 160x160 pixels, with uniformly sampled RGB values. Feature embeddings were then extracted from the generated images with the pre-trained Facenet model (cf. Section~\ref{subsub:face-dataset}). This set of 100,000 raw input vectors, was parsed by a min-max scaler fitted to real user data. We did not align the noisy images, as there is no facial information within the image to align. Note that alignment is normally used in face authentication to detect facial boundaries within an image. \blue{Again, we aggregate results over 50 repetitions to remove any potential biases.}
%\hassan{may be we need to tell people what alignment is}\ben{edited into dataset introduction} %\ben{as such the align pre-processing step fails as there is no facial information contained within the images.}.

The results from these raw inputs are shown in Figure~\ref{fig:face_roc}. We note that the RAR curve behaves much more similarly to the FPR curve, than what was previously observed for raw touch inputs. Also, in the particular example of RBFSVM, we obtain an RAR of 0.09 which is significantly higher than the AR (0.01) at the equal error rate. We again computed the true positive region and found that the average is $6.562 \times 10^{-94} \pm 6.521 \times 10^{-93}$. However, the volume covered by the raw inputs (after feature extraction) is only $4.670 \times 10^{-390}$, which is negligible compared to the ARs (0.15, 0.01, 0.78 and 0.10 for all four classifiers). Additional analysis shows that only one other user's feature space overlapped with the space of raw inputs, with an overlapped area of $8.317 \times 10^{-407}$, many orders of magnitude smaller than both the positive users and the raw feature space itself. \
%hassan{Is this the volume of the intersection, or the true positive region of this particular user?}. \ben{Overlapped would be the intersection, another clarification is that this does not include any user subsampling, just the rectangle size from all the user samples}

\subsection*{Observations} 
The threat of a random input attack via raw random inputs is also high, and in some cases greater than the FPR. However, the region spanned by the feature vectors from these raw inputs is exponentially small and hence does not span the acceptance region. Furthermore, the region also does not coincide with any true positive region. This implies that raw inputs may result in high raw acceptance rate due to the fact that the training data does not have representative vectors in the region spanned by raw inputs. We shall return to this observation when we discuss mitigation strategies in Section~\ref{sec:mitigation}. 


%An additional observation is the rectangular feature space occupied by these raw samples is orders of magnitude smaller than the positive region of any user. Users have an average rectangular space  ($mean \pm SD$), but the volume occupied by the raw inputs only covers $4.670 \cdot 10^{-390}$. Additional analysis shows that only one other user's feature space overlapped with the space of raw inputs ($8.317\cdot 10^{-407}$) many orders of magnitude smaller than both the positive users and the raw feature space itself. The large RAR is counter-intuitive but the smaller area should be easily mitigated with the inclusion of negative samples from said raw area (Section~\ref{sec:mitigation}). Nevertheless we have shown there is a region accessible by random raw inputs that allows attackers to pose as the positive identity.

==> Acceptance Region_camera_ready/mitigation.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Manual placement
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[t]
\caption{Equal Error Rate and AR
%summary between biometric modalities and model architectures 
with and without the mitigation strategy. Green (resp., red) shades highlight improvement (resp., deterioration) in FPR and AR. Color intensity is proportional to degree of performance change.}
%Red shades highlight decreases in performance. Color intensity is proportional to the degree of performance change.}
\label{tab:summary_ar}
\vspace{-0.1cm}
\centering
\resizebox{0.80\textwidth}{!}{%
\begin{tabular}{|l||l|l|l|l||l|l|l|l||l|l|l|l||l|l|l|l|}
\hline
 & \multicolumn{4}{c||}{Linear SVM} & \multicolumn{4}{c||}{Radial Svm} & \multicolumn{4}{c||}{Random Forest} & \multicolumn{4}{c|}{Deep Neural Network} \\ \hline
Biometric & \multicolumn{2}{c|}{Normal} & \multicolumn{2}{c||}{Mitigation} & \multicolumn{2}{c|}{Normal} & \multicolumn{2}{c||}{Mitigation} & \multicolumn{2}{c|}{Normal} & \multicolumn{2}{c||}{Mitigation} & \multicolumn{2}{c|}{Normal} & \multicolumn{2}{c|}{Mitigation} \\ \cline{2-17}
Modality & FPR & AR & FPR & AR & FPR & AR & FPR & AR & FPR & AR & FPR & AR & FPR & AR & FPR & AR \\ \hline
Gait & 0.160 & 0.24 & \cellcolor{red!0} 0.160 & \cellcolor{green!25} 0.04 & 0.140 & 0.18 & \cellcolor{red!0} 0.140 & \cellcolor{green!17.5} 0.04 & 0.09 & 0.03 & \cellcolor{red!0} 0.09 & \cellcolor{green!3.75} 0.00 & 0.215 & 0.20 & \cellcolor{green!5.625} 0.170 & \cellcolor{green!25} 0.00 \\
Touch & 0.325 & 0.49 & \cellcolor{red!1.875} 0.340 & \cellcolor{green!60} 0.01 & 0.265 & 0.41 & \cellcolor{red!0} 0.265 & \cellcolor{green!47.5} 0.03 & 0.21 & 0.23 & \cellcolor{red!0} 0.21 & \cellcolor{green!28.75} 0.00 & 0.325 & 0.30 & \cellcolor{red!6.25} 0.375 & \cellcolor{green!37.5} 0.00 \\
Face & 0.050 & 0.15 & \cellcolor{red!1.875} 0.065 & \cellcolor{green!5} 0.11 & 0.040 & 0.01 & \cellcolor{red!0} 0.040 & \cellcolor{red!0} 0.01 & 0.03 & 0.78 & \cellcolor{red!0} 0.03 & \cellcolor{green!97.5} 0.00 & 0.095 & 0.10 & \cellcolor{green!3.75} 0.065 & \cellcolor{green!7.5} 0.04 \\
Voice & 0.030 & 0.08 & \cellcolor{red!0} 0.030 & \cellcolor{green!2.5} 0.06 & 0.020 & 0.00 & \cellcolor{red!0} 0.020 & \cellcolor{red!0} 0.00 & 0.04 & 0.01 & \cellcolor{red!0} 0.04 & \cellcolor{green!1.25} 0.00 & 0.115 & 0.08 & \cellcolor{green!3.125} 0.090 & \cellcolor{green!7.5} 0.02\\ \hline
\end{tabular}
}
\end{table*}



\begin{table*}[t]
\caption{Equal Error Rate and RAR
%summary between biometric modalities and model architectures 
with and without the mitigation strategy.
%employed on systems subject to RAR. 
The AR values remain the same as in Table~\ref{tab:summary_ar}.
%, and have been excluded from this table. 
$\beta$-RAR 
%under mitigation 
indicates RAR treated with only $\beta$ noise. RAR 
%under Mitigation 
indicates the inclusion of both $\beta$ noise and raw random input samples.}
\label{tab:summary_rar}
\vspace{-0.1cm}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l||l|l|l|l|l||l|l|l|l|l||l|l|l|l|l||l|l|l|l|l|}
\hline
 & \multicolumn{5}{c||}{Linear SVM} & \multicolumn{5}{c||}{Radial Svm} & \multicolumn{5}{c||}{Random Forest} & \multicolumn{5}{c|}{Deep Neural Network} \\ \hline
Biometric & \multicolumn{2}{c|}{Normal} & \multicolumn{3}{c||}{Mitigation} & \multicolumn{2}{c|}{Normal} & \multicolumn{3}{c||}{Mitigation} & \multicolumn{2}{c|}{Normal} & \multicolumn{3}{c||}{Mitigation} & \multicolumn{2}{c|}{Normal} & \multicolumn{3}{c|}{Mitigation} \\ \cline{2-21}
Modality & FPR & RAR & FPR & $\beta$-RAR & RAR & FPR & RAR & FPR & $\beta$-RAR & RAR &  FPR & RAR & FPR & $\beta$-RAR & RAR &  FPR & RAR & FPR & $\beta$-RAR & RAR \\ \hline
Touch Raw & 0.325 & 0.45 & \cellcolor{red!2.5} 0.345 & \cellcolor{green!1.25} 0.44 & \cellcolor{green!56.25} 0.00 & 0.265 & 0.40 & \cellcolor{red!0} 0.265 & \cellcolor{green!5} 0.36 & \cellcolor{green!48.75} 0.01 & 0.21 & 0.18 & \cellcolor{red!0.625000000000001} 0.215 & \cellcolor{green!16.25} 0.05 & \cellcolor{green!22.5} 0.00 & 0.325 & 0.32 & \cellcolor{red!6.875} 0.38 & \cellcolor{green!7.5} 0.26 & \cellcolor{green!40} 0.00 \\
Face Raw & 0.050 & 0.12 & \cellcolor{red!3.125} 0.075 & \cellcolor{red!2.5} 0.14 & \cellcolor{green!15} 0.00 & 0.040 & 0.09 & \cellcolor{red!0} 0.040 & \cellcolor{red!0} 0.09 & \cellcolor{green!11.25} 0.00 & 0.03 & 0.02 & \cellcolor{red!0} 0.030 & \cellcolor{green!1.25} 0.01 & \cellcolor{green!2.5} 0.00 & 0.095 & 0.10 & \cellcolor{green!3.125} 0.07 & \cellcolor{green!5} 0.06 & \cellcolor{green!8.75} 0.03\\ \hline
\end{tabular}
}
\vspace{-0.2cm}
\end{table*}



\section{Mitigation}
\label{sec:mitigation}
In the previous section, we validated that higher variance in the samples in the negative class as compared to the variance of samples from the target user class reduces AR. The data from the negative class is obtained from real user samples, and therefore scheme designers cannot control the variance. However, this gives us a simple idea to minimize AR: generate noise vectors around the target user's vectors and treat it as part of the negative class for training the model. This will result in the tightening of the acceptance region around the true positive region. We remark that the noise generated is independent of the negative training samples.

% \paragraph{Higher Variance Synthetic samples in the Training set}

% It was previously observed in Section \ref{sec:synthetic_isolate}, that the relative difference in feature variance between a user's own samples and negative training samples have a direct impact on the Acceptance Region of the resulting model. With this observation we investigate the possibility of including a negative synthetic dataset randomly sampled with higher variance than the user's own features. We have balanced the training and testing data between the positive and negative class, ensuring testing completeness through repetition. Departing from this notion, we include an additional set of training samples balanced in size to both the user's positive, and the population negative samples. The training set remains balanced with a 1/3rd of the training samples originating from each source.


% --Side note:
% There is no obligation to use real negative samples as provided from the users, we can fit normal distributions into the user features, and re-sample new negative samples around the original mean, but with a increased amount of standard deviation depended on the positive user.

% \ben{pending test, assumes the trainer has statistics from other users in the training set.}



\subsection{The Beta Distribution}
More specifically, we generate additional negative training samples by sampling noisy vectors where each feature value is sampled from a beta distribution. We generate samples equal to the number of samples in the positive class. Thus creating a dataset with a third of the samples as positive, another third as negative samples from other users, and finally the remaining third of feature vectors treated as negative samples from the beta distribution dependent on the positive user. The procedure is as follows. For the $i$th feature, let $\mu_i$ denote the mean value for the given target user. We use the beta distribution with parameters $\alpha_i = | 0.5 - \mu_i| + 0.5$ and $\beta_i = 0.5$. We denote the resulting beta distribution by $\mathcal{B}e(\alpha_i, \beta_i)$. Then a noisy sample $\mathbf{x}$ is constructed by sampling its $i$th element $x_i$ from the distribution $ \mathcal{B}e(\alpha_i, \beta_i)$ if $\mu_i \le 0.5$, and from $1 - \mathcal{B}e(\alpha_i, \beta_i)$ otherwise. The two cases ensure that we add symmetric noise as the mean moves over to either side of $0.5$. 


% This beta distribution however will be skewed to either extreme of the feature space depending on the mean of the positive samples. 


% The beta-distribution we use has parameters: $\alpha_i = |E(f_{i, u}) - 0.5| + 0.5$ and $\beta_i=0.5$, where $E(f_{i, u})$ is the mean of a feature dimension for the positive training samples. Finally the noise $ = | -1*\lfloor E(f_{i, u})\rceil + B(\alpha_i, \beta_i)|$

% \hassan{What shape are we expecting here?} \ben{I read somewhere that $\lfloor x \rceil$ means round $x$ to the nearest integer, is this consistent with your understanding?}

%\subsection*{Results on AR}
\descr{Results on AR.} In Table \ref{tab:summary_ar}, we show the resulting FPR and AR after the addition of beta noise at the equal error rate. The detailed ROC curves are shown in Figure~\ref{fig:all_beta_def} in Appendix~\ref{sec:mitigation_roc}. In every configuration (classifier-dataset pairs), we see a significant decrease in AR. The AR is now lower than FPR in every configuration. In 14 out of 16 cases, the AR is $\le 0.04$. The two exceptions are LinSVM (with face and voice datasets). We further see that in 13 out of 16 instances the FPR either remains unchanged or improves! The 3 instances where the FPR degrades are LinSVM with face and face datasets both by $+0.015$, and DNN with Touch where the difference is $+0.05$. Thus, adding beta distributed noise does indeed decrease the AR with minimal impact on FPR. This agrees with our postulate that high AR was likely due to loose decision boundaries drawn by the classifier, and the addition of beta noise tightens this around the true positive region. Figure \ref{fig:individual_ar-fpr_def} in Appendix~\ref{sec:mitigation_roc} displays individual user FPRs and ARs.

% \ref{fig:gait_beta_def}, \ref{fig:face_beta_def}, \ref{fig:touch_beta_def}, \ref{fig:voice_beta_def}
% , and Table \ref{tab:summary_ar}, we can observe the addition of additional samples from a beta distribution yields improvements on the AR performance of the system, bringing AR performance below the relatively unchanged FPR, in most cases with the exception of Linear SVM when the starting FPR was already low. This test simply adds beta distribution noise to the training set, that is only dependent on the statistics of the user's own training samples (positive class), and thus will scale to systems of more users.

% In all classifiers with respect to AR, we strictly observe improvements to the AR (lower AR), with a few classifiers being able to completely repel the uniformly generated samples. The FPR of the schemes remain relatively unchanged from before the noise was added (with the exception of 3 instances, 2 from Touch, 1 from Face). This unchanging FPR agrees with the original intuition of the attack and the subsequent addition of beta-distributed noise as we speculated that there may be regions of the feature space distant from the decision boundary still considered as positive, thus by adding beta-distributed noise concentrated in the edges of the feature space, the boundary should remain relatively unchanged. The full ROC behaviours can be found in Appendix~\ref{sec:mitigation_roc}.





% \begin{table*}[t]
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{|l||l|l|l|l||l|l|l|l||l|l|l|l||l|l|l|l|}
% \hline
%  & \multicolumn{4}{c||}{Linear SVM} & \multicolumn{4}{c||}{Radial Svm} & \multicolumn{4}{c||}{Random Forest} & \multicolumn{4}{c|}{Deep Neural Network} \\ \hline
% Biometric & \multicolumn{2}{l|}{Normal} & \multicolumn{2}{l||}{Mitigation} & \multicolumn{2}{l|}{Normal} & \multicolumn{2}{l||}{Mitigation} & \multicolumn{2}{l|}{Normal} & \multicolumn{2}{l||}{Mitigation} & \multicolumn{2}{l|}{Normal} & \multicolumn{2}{l|}{Mitigation} \\ \cline{2-17}
% Modality & FPR & AR & FPR & AR & FPR & AR & FPR & AR & FPR & AR & FPR & AR & FPR & AR & FPR & AR \\ \hline
% Gait & 0.160 & 0.24 & \cellcolor{red!0} 0.160 & \cellcolor{green!25} 0.04 & 0.140 & 0.18 & \cellcolor{red!0} 0.140 & \cellcolor{green!17.5} 0.04 & 0.09 & 0.03 & \cellcolor{red!0} 0.09 & \cellcolor{green!3.75} 0.00 & 0.215 & 0.20 & \cellcolor{green!5.625} 0.170 & \cellcolor{green!25} 0.00 \\
% Touch & 0.325 & 0.49 & \cellcolor{red!1.875} 0.340 & \cellcolor{green!60} 0.01 & 0.265 & 0.41 & \cellcolor{red!0} 0.265 & \cellcolor{green!47.5} 0.03 & 0.21 & 0.23 & \cellcolor{red!0} 0.21 & \cellcolor{green!28.75} 0.00 & 0.325 & 0.30 & \cellcolor{red!6.25} 0.375 & \cellcolor{green!37.5} 0.00 \\
% Face & 0.050 & 0.15 & \cellcolor{red!1.875} 0.065 & \cellcolor{green!5} 0.11 & 0.040 & 0.01 & \cellcolor{red!0} 0.040 & \cellcolor{red!0} 0.01 & 0.03 & 0.78 & \cellcolor{red!0} 0.03 & \cellcolor{green!97.5} 0.00 & 0.095 & 0.10 & \cellcolor{green!3.75} 0.065 & \cellcolor{green!7.5} 0.04 \\
% Voice & 0.030 & 0.08 & \cellcolor{red!0} 0.030 & \cellcolor{green!2.5} 0.06 & 0.020 & 0.00 & \cellcolor{red!0} 0.020 & \cellcolor{red!0} 0.00 & 0.04 & 0.01 & \cellcolor{red!0} 0.04 & \cellcolor{green!1.25} 0.00 & 0.115 & 0.08 & \cellcolor{green!3.125} 0.090 & \cellcolor{green!7.5} 0.02\\ \hline
% \end{tabular}
% }
% \vspace{0.1cm}
% \caption{Equal Error Rate summary between biometric modalities and model architectures with and without the mitigation strategy employed. Highlighted in green is a improvement in the rejection of the negative samples, weather that is from other users (FPR), smaller Acceptance Regions (AR). Highlighted in red is decreases in performance. The colour intensity is proportional to the degree of performance change.}
% \label{tab:summary_ar}
% \end{table*}



% \begin{table*}[t]
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{|l||l|l|l|l|l||l|l|l|l|l||l|l|l|l|l||l|l|l|l|l|}
% \hline
%  & \multicolumn{5}{c||}{Linear SVM} & \multicolumn{5}{c||}{Radial Svm} & \multicolumn{5}{c||}{Random Forest} & \multicolumn{5}{c|}{Deep Neural Network} \\ \hline
% Biometric & \multicolumn{2}{l|}{Normal} & \multicolumn{3}{l||}{Mitigation} & \multicolumn{2}{l|}{Normal} & \multicolumn{3}{l||}{Mitigation} & \multicolumn{2}{l|}{Normal} & \multicolumn{3}{l||}{Mitigation} & \multicolumn{2}{l|}{Normal} & \multicolumn{3}{l|}{Mitigation} \\ \cline{2-21}
% Modality & FPR & RAR & FPR & $\beta$-RAR & RAR & FPR & RAR & FPR & $\beta$-RAR & RAR &  FPR & RAR & FPR & $\beta$-RAR & RAR &  FPR & RAR & FPR & $\beta$-RAR & RAR \\ \hline
% Touch Raw & 0.325 & 0.45 & \cellcolor{red!2.5} 0.345 & \cellcolor{green!1.25} 0.44 & \cellcolor{green!56.25} 0.00 & 0.265 & 0.40 & \cellcolor{red!0} 0.265 & \cellcolor{green!5} 0.36 & \cellcolor{green!48.75} 0.01 & 0.21 & 0.18 & \cellcolor{red!0.625000000000001} 0.215 & \cellcolor{green!16.25} 0.05 & \cellcolor{green!22.5} 0.00 & 0.325 & 0.32 & \cellcolor{red!6.875} 0.38 & \cellcolor{green!7.5} 0.26 & \cellcolor{green!40} 0.00 \\
% Face Raw & 0.050 & 0.12 & \cellcolor{red!3.125} 0.075 & \cellcolor{red!2.5} 0.14 & \cellcolor{green!15} 0.00 & 0.040 & 0.09 & \cellcolor{red!0} 0.040 & \cellcolor{red!0} 0.09 & \cellcolor{green!11.25} 0.00 & 0.03 & 0.02 & \cellcolor{red!0} 0.030 & \cellcolor{green!1.25} 0.01 & \cellcolor{green!2.5} 0.00 & 0.095 & 0.10 & \cellcolor{green!3.125} 0.07 & \cellcolor{green!5} 0.06 & \cellcolor{green!8.75} 0.03\\ \hline
% \end{tabular}
% }
% \vspace{0.1cm}
% \caption{Equal Error Rate summary between biometric modalities and model architectures with and without the mitigation strategy employed on systems subject to RAR. The AR values remain the same as those in Table~\ref{tab:summary_ar}, and have been excluded from this table. $\beta$-RAR under the mitigation indicates the RAR of the models treated with only $\beta$ noise, RAR under Mitigation indicates the inclusion of both $\beta$ noise and samples from the RAR region.}
% \label{tab:summary_rar}
% \end{table*}



%\subsection*{Results on RAR}
\descr{Results on RAR.} %\paragraph{Faux Raw Extracted Features}
%Previously in Section~\ref{sec:classify_face} and \ref{sec:classify_touch}, we observed a substantial proportion of vectors extracted from fabricated raw inputs were granted access to the system by the biometric model. 
Interestingly, beta distributed noise only marginally reduces the raw acceptance rate as can be seen in Table~\ref{tab:summary_rar} (columns labeled $\beta$-RAR). 
%The aforementioned beta distributed noise, while effective in mitigating the AR of uniformly samples attack vectors, did not effectively prevent attacks using raw extracted features from gaining access as noted in Table~\ref{tab:summary_rar}. 
The reason for this lies in the volume of the region spanned by random raw inputs. We previously saw in Section~\ref{sub:rar-results} that it was (a) exponentially small and (b) many orders of magnitude smaller than the true positive region. Thus, it is unlikely that beta distributed noise will lie in this region to aid the model to label them as negative samples. Consequently we sought another means to mitigate this attack surface. 
%, as the raw-input attack is still shown to be effective in gaining a positive response from user models.

%\vspace{-2mm}
\subsection{Feature Vectors from Raw Inputs as Negative Samples}
%\ben{Possibility of measuring region overlap in a centroid based measure.}
%\ben{Results of RAR with only the beta-defence included within appendix, quote and ref in text is ideal solution}
Our mitigation strategy to reduce RAR is to include a subset of raw input vectors in the training process, whose cardinality is equal to the number of positive user samples in the training dataset. The training dataset now contains 1/4th each of raw input vectors, beta-noise, positive samples, and samples from other users.   

%The user's positive samples in conjunction with the negative samples of raw input vectors, beta-noise, and other user data will each contribute 1/4 of the training set. 

%\subsection*{Results on AR and RAR}
\descr{Results on AR and RAR.}
Table~\ref{tab:summary_rar} shows that the mitigation strategy reduces the RAR to less than or equal to 0.03 in all instances (columns labeled RAR). The resulting FPR is marginally higher than the FPR from only beta-distributed noise in some cases (Table~\ref{tab:summary_ar}). Thus, the inclusion of beta-distributed noise in conjunction with subset of raw inputs in the training data reduces both AR and RAR with minimal impact on FPR and FRR. 



% With only beta-noise we observed there was a minimal impact to the FPR and TPR of the system, with a substantial reduction of the uniform vector AR. This however was not sufficient to reduce the RAR, by introducing additional negative samples generated directly from the raw generated inputs, we are able to reject near all of these test samples. However, following our hypothesis that RAR is closer to the feature space of genuine samples, we observe a small percentage increase in the error rates of the classifier when testing genuine biometrics. A summary of these changes can be found in Table~\ref{tab:summary_rar}. To put the effectiveness of the additional negative samples into perspective, 1M uniform vectors targeting the AR are being effectively thwarted by the inclusion an average 240 for gait, 2567 for touch, 313 for face, and 284 for voice. Likewise, the RAR of 100K raw inputs are thwarted by an equivalent number.

% \hassan{Out of curiosity, we couldn't we use random feature vectors as a mitigation measure for AR?}
% \ben{One objective was to minimize the impact on the regular behaviour of the model, i.e. under typical use the model is unaffected. If it is argued AR is an edge case we can also present that the mitigation strategy is basically free, so who not include it?}

% \hassan{I think adding random feature vectors as negative class to reduce AR would effect FRR and FPR, as they would span all over the feature space.}


% \section{Faux Raw Extracted Features}

% By sampling uniform vectors from the feature space we have shown that an attacker is able to gain access at a sufficient rate with little to no cost. A more realistic attack scenario is if an attacker only has access to the system before the feature extraction process. As such we test the capability of an attacker with minimal knowledge of the biometric process in generating the raw inputs.

% A minimal amount of knowledge for an attacker in a facial authentication system is knowing only the size of the image, disclosed (and enforced) if the feature extraction process only accepts inputs of a fixed size. With this information, the attacker with no other knowledge and assumptions can effectively generate noise.

% \begin{figure*}[th!]
% 	\centering
%     \includegraphics[width=1.0\textwidth]{images/gait_betadefence_roc-crop.pdf}
%   	\caption{Gait beta-noise mitigation results, with training noise sampled from a symmetric beta distribution the EER is marked on the diagrams. %\red{This is ideal performance, FPR's unchanged, and AR is substantially lower.}
%   	}
%  	\label{fig:gait_beta_def}
% \end{figure*}

% \begin{figure*}[th!]
% 	\centering
%     \includegraphics[width=1.0\textwidth]{images/face_betadefence_roc-crop.pdf}
%   	\caption{Face beta-noise mitigation results, with training noise sampled from a symmetric beta distribution the EER is marked on the diagrams. %\red{great improvement on the AR, and minor improvements for the FPR}
%   	}
%  	\label{fig:face_beta_def}
% \end{figure*}

% \begin{figure*}[th!]
% 	\centering
%     \includegraphics[width=1.0\textwidth]{images/touch_betadefence_roc-crop.pdf}
%   	\caption{Touch beta-noise mitigation results, with training noise sampled from a symmetric beta distribution the EER is marked on the diagrams. %\red{great improvement on the AR, and minor decrease in the FPR performance}
%   	}
%  	\label{fig:touch_beta_def}
% \end{figure*}

% \begin{figure*}[th!]
% 	\centering
%     \includegraphics[width=1.0\textwidth]{images/voice_betadefence_roc-crop.pdf}
%   	\caption{Voice beta-noise mitigation results, with training noise sampled from a symmetric beta distribution the EER is marked on the diagrams. %\red{minor improvement on AR, LIN svm AR still above FPR, additionally NN FPR performance has improved}
%   	}
%  	\label{fig:voice_beta_def}
% \end{figure*}


% \begin{table*}[t]
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{|l||l|l|l|l||l|l|l|l||l|l|l|l||l|l|l|l|}
% \hline
% EERs & \multicolumn{4}{c||}{Linear SVM} & \multicolumn{4}{c||}{Radial Svm} & \multicolumn{4}{c||}{Random Forest} & \multicolumn{4}{c|}{Deep Neural Network} \\ \hline
% Biometric & \multicolumn{2}{l|}{Normal} & \multicolumn{2}{l||}{Mitigation} & \multicolumn{2}{l|}{Normal} & \multicolumn{2}{l||}{Mitigation} & \multicolumn{2}{l|}{Normal} & \multicolumn{2}{l||}{Mitigation} & \multicolumn{2}{l|}{Normal} & \multicolumn{2}{l|}{Mitigation} \\ \cline{2-17}
% Modality & FPR & AR & FPR & AR & FPR & AR & FPR & AR & FPR & AR & FPR & AR & FPR & AR & FPR & AR \\ \hline
% Gait & 0.15 & 0.22 & 0.15 & \cellcolor{green!36}0.04 & 0.14 & 0.17 & 0.14 & \cellcolor{green!18}0.05 & 0.09 & 0.09 & 0.09 & \cellcolor{green!16}0.01 & 0.16 & 0.16 & 0.16 & \cellcolor{green!32}0.00 \\ \hline
% Face & 0.05 & 0.14 & \cellcolor{red!06}0.06 & \cellcolor{green!08}0.10 & 0.04 & 0.03 & 0.04 & \cellcolor{green!04}0.02 & 0.04 & 0.08 & \cellcolor{green!3}0.03 & \cellcolor{green!10}0.03 & 0.10 & 0.08 & \cellcolor{green!12}0.06 & \cellcolor{green!06}0.06 \\ \hline
% Touch & 0.29 & 0.47 & \cellcolor{red!9}0.31 & \cellcolor{green!90}0.02 & 0.26 & 0.40 & 0.26 & \cellcolor{green!72}0.04 & 0.20 & 0.20 & 0.20 & \cellcolor{green!38}0.01 & 0.32 & 0.30 & \cellcolor{red!15}0.37 & \cellcolor{green!60}0.00 \\ \hline
% Voice & 0.03 & 0.06 & 0.03 & \cellcolor{green!04}0.04 & 0.02 & 0.01 & 0.02 & 0.01 & 0.06 & 0.06 & \cellcolor{green!06}0.04 & \cellcolor{green!08}0.02 & 0.11 & 0.09 & \cellcolor{green!9}0.08 & \cellcolor{green!06}0.06 \\ \hline
% \end{tabular}
% }
% \caption{\red{OLD TABLE}Equal Error Rate summary between biometric modalities and model architectures with and without the mitigation strategy employed. Highlighted in green is a improvement in the rejection of the negative samples, weather that is from other users (FPR), smaller Acceptance Regions (AR). Highlighted in red is decreases in performance. The colour intensity is proportional to the degree of performance change.}
% \label{tab:summary}
% \end{table*}











% \paragraph{Sampling from the positive user's normal distribution, with 30\% increased standard deviation}
% The figure Below displays a negative affect on AR and FPR in the case of facenet.
% Logically this is an expected outcome as creating negative samples from your own user's statistics will place a large number of negative samples is a space that was previously dominated by positive samples, thus decreasing the certainty for the ML algorithm.
% \ben{Tried it on facenet, detrimental to performance for all classifiers except Radial SVM, do no proceed with this test.}

% \begin{figure*}[th!]
% 	\centering
%     \includegraphics[width=1.0\textwidth]{images/face_defence_roc.pdf}
%   	\caption{\red{Face authentication results, with training noise sampled from the positive user statistics. the EER is marked on the diagrams. NOT THE WAY FORWARDS}}
%  	\label{fig:face_def}
% \end{figure*}



% \paragraph{Biometric Key Generation}
% By offloading the fuzzy to another module,  
%\subsection{A Secure Mobile Authentication Alternative to Biometrics}
%\red{Will not work, due to protection offered by random projections}
%We test our idea on Azimpourkivi's ai.lock \cite{azimpourkivi2017secure}. We redeploy the code as provided in their paper, training only on the nexus image dataset (features have been pre-extracted from the Inception deep learning model). We then modify their test script to receive noise as the input vector, instead of an image's feature vector. Upon rerunning their system and with their optimized threshold, we obtain performance results of: TPR, FPR, FNR, TNR. After testing random attacks against all users, we obtain a Acceptance region of XXXX. The way we generate the noise is by creating a binary vector of equal length to the system input, and randomly populating it with 0s and 1s.

==> Acceptance Region_camera_ready/synthetic.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Synthetic Dataset}
\label{sec:synthetic}

\begin{figure*}[th!]
	\centering
    \includegraphics[width=1.0\textwidth]{images/isolate_user_variance-crop.pdf}
    \vspace{-0.65cm}
  	\caption{A comparison between FPR, AR, four different ML architectures. Trained on synthetic data of 50 features of 50 user, of increasing variance within features for a singular user, repeated 50 times. Note how the system level AR and FPR remains unchanging, despite the isolated user's AR increasing substantially.}
 	\label{fig:isolate_userv}
 	\vspace{-0.10cm}
\end{figure*}

\begin{figure*}[th!]
	\centering
    \includegraphics[width=1.0\textwidth]{images/isolate_other_variance-crop.pdf}
    \vspace{-0.65cm}
  	\caption{A comparison between FPR, AR, four different ML architectures. Trained on synthetic data of 50 features of 50 user, of increasing variance within features of all other users except a singular user, repeated 50 times. The x-axis denotes the relative SD of the population compared with the isolated user.}
 	\label{fig:isolate_otherv}
 	\vspace{-0.05cm}
\end{figure*}

%In the previous section, we saw that for some dataset-classifier pairs, AR is significantly higher than FPR, and even in cases where the average AR is comparable to the average FPR, per-user ARs can be significantly higher and often unrelated to FPR. However, 
The analysis in the previous section was limited in the sense that we could not isolate the reasons behind the discrepancy between AR and FPR. Indeed, we saw that for some configurations (dataset-classifier pairs), the AR curve nicely followed the FPR curve, e.g., the face dataset and DNN (Figure~\ref{fig:face_ind}), where as for others this was not the case. In order to better understand the factors effecting AR, in this section we attempt to empirically verify the hypothesized factors effecting the acceptance region outlined in Section~\ref{sec:attack_def}. Namely, high feature variance in a target user's samples is likely to increase AR, and low feature variance in the user samples in the negative class is expected to result in high AR. In both these cases, we expect to achieve a reasonably low EER, but AR may still be significantly greater than FPR. Moreover, if these factors are indeed true, we expect to see similar behavior across all classifiers. To test this we create a synthetic model of a biometric dataset. 
%With this synthetic biometric dataset we evaluate how the variance of features in the target user and the users in the negative class impacts the acceptance region of the resulting user models.


%As described in Section~\ref{sec:attack_def}, the distribution and separation of the datasets within the feature space will effect the resulting decision boundary; and hence the proportion of feature space accepted as the positive region. In section \ref{sec:realscheme} we observed that there is a measurable space in which uniformly generated samples are incorrectly verified by user models trained on real-world data through these positive regions. This acceptance region is considerable, despite a reasonable EER-FPR chosen with the employ of best practice. In this section we aim to understand how dataset variables can influence the size of the positive region. We experiment with a 



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Manual placement
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\subsection{Simulating a Biometric Dataset}
Let $\mathcal{N}(\mu, \sigma^2)$, denote the normal distribution with mean $\mu$ and standard deviation $\sigma$. We assume each feature to be normally distributed across all users with slight variations in mean and standard deviation across all features and users. More specifically, our methodology for generating the synthetic dataset is as follows.
\begin{enumerate}[leftmargin=5mm]
    \item We model the mean of all $n$ features taking values in the unit interval $\mathbb{I}$ as a normally distributed random variable $\mathcal{N}(\mu_{\text{mn}}, \sigma^2_{\text{mn}}) = \mathcal{N}(0.5, 0.1^2)$. Similarly we model the standard deviation of all $n$ features as another normally distributed random variable $\mathcal{N}(\mu_{\text{var}}, \sigma^2_{\text{var}}) = \mathcal{N}(0.1, 0.07^2)$. 
    \item For each feature $i \in [n]$, we first sample $\mu_i \leftarrow \mathcal{N}(\mu_{\text{mn}}, \sigma^2_{\text{mn}})$ and $\sigma_i \leftarrow \mathcal{N}(\mu_{\text{var}}, \sigma^2_{\text{var}})$. The resulting normal distribution $\mathcal{N}(\mu_{i}, \sigma^2_{i}) $ serves as the population distribution of the mean of the feature $i$.
    \item For each user $u$, we sample the mean $\mu_{u, i} \leftarrow \mathcal{N}(\mu_{i}, \sigma^2_{i})$. The variance $\sigma^2_{u, i}$ is chosen as the control variable. User $u$'s samples for the $i$th feature are generated as i.i.d. random variables $\mathcal{N}(\mu_{u, i}, \sigma^2_{u, i})$, which serves as user $u$'s distribution for the $i$th feature. 
\end{enumerate}
 

% In a biometrics dataset of users performing a similar action (behavioural biometric), or recording a specific body-part (physiological biometric), every user can be fit into a distribution of features (we assume a Gaussian distribution), termed the population statistics. These global parameters allow for the creation of a random user by sampling with a given feature mean within the population.
% \vspace{-\topsep}
% \begin{itemize}
%   \item The mean for a feature of random user, can be sampled from the population statistics.
% \end{itemize}
% \vspace{-\topsep}
% Additionally users performing biometrics will inadvertently generate varied samples, the degree of variation is dependent on the individual user; like the feature means, there will be a distribution of variances within the population.
% \begin{itemize}[noitemsep,topsep=0pt]
%   \item The standard deviation for a feature of random user, can be sampled from the population statistics. 
% \end{itemize}
% Once the feature mean and standard deviation for a generated user has been created from the population statistics, a dataset for the given user can be sampled. 
% \begin{itemize}[noitemsep,topsep=0pt]
%   \item A collection of feature samples from a random user, can be sampled from the previously generated set of distribution parameters. 
% \end{itemize}



% The creation of every set of user parameters is I.I.D from the population statistics, with the user's subsequent samples I.I.D from the distributions defined by the parameters. This provides a basis for rapidly evaluating dependencies between the dataset and the Acceptance region. 

% As the feature mean itself is a distribution, We sampled the mean of the feature mean from a Gaussian with $0.5 \pm 0.1$, and the SD of the feature mean was sampled from another Gaussian distribution with a mean and SD of $0.1 \pm 0.07$. The feature mean and SD are sampled anew for all features to produce a semi-unique mean distribution for each feature.

%In regards to the feature variance, it can also be represented by a distribution with a mean and SD. However as we plan to tightly control this variable, the exact distribution depends on the exact experiment. 
We evaluate the same four types of ML architectures, LinSVM, RBFSVM, RNDF and DNN. Due to the large number of potential configurations we evaluate the model performance at a fixed threshold of 0.5. For the experiments we choose 50 (synthetic) users, with 50 features in the feature space. Each experimental run is repeated 50 times \blue{to reduce any potential biases arising from the random process.}  

% \subsection{Classifier Construction}

% \hassan{The following is redundant}

% In this section, we evaluate the same 4 types of ML architectures, Linear SVM (LSVM), Radial SVM (RSVM), Random Forests (RNDF) and a Deep Neural Network (DNN).

% Every ML model is configured for Binary Classification (the returning user, or not). The training of these models use a positive class from the returning user's own samples, and a negative class, evenly sampled from the other users in the study. We balance the number of training samples from the positive and the negative class to avoid training bias and over-fitting any one class. The feature-set is min-max normalized across the entire dataset prior to being split 70\%-30\% per user for training and testing. 





% \subsection{Acceptance Region}
% To measure the Acceptance Region of the trained model, we uniformly sample 1 Million test samples from the feature space. These samples are then passed to the model to be classified, the proportion of the random test samples incorrectly accepted as positive out of all generated test samples is the Acceptance Region of the model.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Results}
% For the first experiment we vary the number of features within the dataset, followed by varying the effect of number of users within the dataset. For every variation of the dataset, we repeat the experiment 50 times, and display the metric mean across all users within the experiment.

% \subsubsection{Varying Number of Features}
% Our simulated dataset is generated 5 times, each with a different number of features, from 10 to 50, in increments of 10.

% Figure \ref{fig:vary_features} displays the average False Positive Rate (FPR) and the Acceptance Region (AR) of the ML models, it can be observed that the AR of these models are consistently larger than the FPR obtained in a zero-effort attack. With an increasing number of features, more information about each user is available, Thus as expected, both the FPR and AR approaches zero. 

% % \hassan{The acceptance region goes down too. What is our benchmark? $c^{-d}$, where $d$ is the number of features and $c < 1$ is some constant? Are we expecting a negligible region?}
% % \ben{Thoughts about $c$, c should describe the known overlap between the positive class and the negative class, likely related to the variance between them. we randomly sample a mean, and also randomly sample a variance. the overlap between the positive class and the negative class should on average just be the mean variance in which we sample features. (some will have more, some less depending on the sampled mean, and sampled variance.). So if that makes sense, $c = 0.2$, which should produce a negligible baseline.}
% % \ben{The alternative way to think about this is for an given $c<1$, we should be expecting a negligible overlap between the positive and negative samples, however whilst the ML model can learn to effectively separate the training data, it also attempts to generalize the two classes to handle unseen data, which leads to a non-negligible area for both FPR and AR.}

% \begin{figure*}[th!]
% 	\centering
%     \includegraphics[width=1.0\textwidth]{synthetic_vary_nfeats-crop.pdf}
%     \vspace{-0.5cm}
%   	\caption{A comparison between FPR and AR of four different ML architectures. Trained on synthetic data of 50 users, with a variable number of features, repeated 50 times.}
%  	\label{fig:vary_features}
% \end{figure*}




% \subsubsection{Varying Number of Users}
% In this test we increase the number of users within the synthetic dataset, testing between 25 to 150, in increments of 25.

% In Figure \ref{fig:vary_users}, we can observe that with the addition of more users into the dataset, the FPR of the system increases. This is expected as the likelihood of user features being similar between any two users increase with more users in the population. As the training of the classifier uses samples from other users as a negative class, the increased number of negative users lowers the AR of the classifier, likely due to the increased variation of the negative training set with additional users sufficiently covering more of the feature space.

% %\hassan{Once again AR is higher than FPR. Why would this be related to the birthday problem?} \ben{The birthday problem states that in a room of people, the probability that two users have the same birthday increases exponentially. In the case of the FPR of our authentication system, the probability that another user has a similar biometric profile/sample to our target user also increases exponentially.}

% \begin{figure*}[th!]
% 	\centering
%     \includegraphics[width=1.0\textwidth]{synthetic_vary_nusers-crop.pdf}
%     \vspace{-0.5cm}
%   	\caption{A comparison between FPR and AR of four different ML architectures. Trained on synthetic data of 50 features per user, with a variable number of users, repeated 50 times.}
%  	\label{fig:vary_users}
% \end{figure*}
% %%%
% % \hassan{I am not sure if 50 features per user is common? Can we use a more typical number?}\ben{It would be hard to definitively say what a typical number of features is, as later in the Facial authentication section, each face image has 512 features, and 1024 for Voice authentication.}\ben{It will also be a good idea to use a smaller number of features, to visually show a larger variation in the FPRs and ARs, when we change the number of users.}
% %%%


% \subsubsection{Changing Variance of User features.}
% \label{sec:synthetic:var}

% When sampling our synthetic dataset, we have previously also sampled the user feature variance, in this test we fix 50 users, and 50 features, but vary the standard deviation from which the synthetic data is sampled.

% Figure \ref{fig:vary_user_feat} demonstrates the expected result that with increasing feature variance, the TPR and FPR performance of the classifier will decrease, as the task of separating the positive and negative classes becomes more difficult. AR on the other hand is observed to have increased, again likely due to the the classifier needing to accept a larger region to encompass the more varied positive samples.

% %In addition to observing an AR larger than the FPR, it is observed in Figure \ref{fig:vary_user_feat} that within a set of user's some users will have a larger AR. An increased variance in the user feature, in particular those deemed important by the training process, is likely to leave a larger surface in which samples are accepted.

% \begin{figure*}[th!]
% 	\centering
%     \includegraphics[width=1.0\textwidth]{synthetic_vary_vfeat-crop.pdf}
%     \vspace{-0.5cm}
%   	\caption{A comparison between FPR, AR, and TPR of four different ML architectures. Trained on synthetic data of 50 features of 50 user, of increasing variance within features, repeated 50 times.}
%  	\label{fig:vary_user_feat}
% \end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{figure*}[th!]
% 	\centering
%     \includegraphics[width=1.0\textwidth]{images/isolate_user_variance-crop.pdf}
%     \vspace{-0.5cm}
%   	\caption{A comparison between FPR, AR, four different ML architectures. Trained on synthetic data of 50 features of 50 user, of increasing variance within features for a singular user, repeated 50 times. Note how the system level AR and FPR remains unchanging, despite the isolated user's AR increasing substantially.}
%  	\label{fig:isolate_userv}
% \end{figure*}

% \begin{figure*}[th!]
% 	\centering
%     \includegraphics[width=1.0\textwidth]{images/isolate_other_variance-crop.pdf}
%     \vspace{-0.5cm}
%   	\caption{A comparison between FPR, AR, four different ML architectures. Trained on synthetic data of 50 features of 50 user, of increasing variance within features of all other users except a singular user, repeated 50 times. The x-axis denotes the relative SD of the population compared with the isolated user.}
%  	\label{fig:isolate_otherv}
% \end{figure*}

\blue{
\begin{figure*}[th!]
	\centering
    \includegraphics[width=1.0\textwidth]{images/synth_cosine_roc-crop.pdf}
    \vspace{-0.7cm}
  	\caption{\blue{ROC Curves versus the AR curve for different ML architectures, including a cosine similarity distance-based classifier. Trained on synthetic data of 50 features of 50 user, with fixed mean and variance for features of all users, repeated 50 times.}}
 	\label{fig:cosine_results}
 	\vspace{-0.1cm}
\end{figure*}

\begin{figure*}[th!]
	\centering
    \includegraphics[width=1.0\textwidth]{images/synthetic_vary_nusers-crop.pdf}
    \vspace{-0.6cm}
  	\caption{\blue{A comparison between FPR and AR of four different ML architectures. Trained on synthetic data of 50 features per user, with a variable number of users, repeated 50 times.}}
 	\label{fig:vary_users}
 	\vspace{-0.2cm}
\end{figure*}
}

\subsection{Effects of Feature Variance on Acceptance Region}
\label{sub:eff-var}
%A machine learning model aims to include as many positive samples within the positive region, and as many negative samples in the negative region as possible. Given our use of a balanced dataset, neither is favoured. As such it is speculated that is a specific user's features are more varied, the machine learner will decide on a boundary encompassing a larger region, which will result in a larger AR.

\subsubsection{Variable Isolated User Variance and Fixed Population Variance}



We first treat one out of the 50 users as an outlier, whcih we call the \emph{isolated} user. %The rest of the users have the same feature variance. %\hassan{We need to use notation defined in subsection A}
%Thus For this experiment, we retain the previous test configuration with 50 users, 50 features, repeated 50 times per change in our specific user's variance. 
The variance $\sigma^2_{u, i}$ is fixed at $(0.2)^2$ for all other users $u$ and for all features $i \in [n]$. We vary the variance $\sigma_{u_\text{tgt}, i}$ of the isolated user $u_\text{tgt}$ from 0.05 to 0.35 in increments of 0.05. Figure~\ref{fig:isolate_userv} plots the user's standard deviation $(\sigma_{u_\text{tgt}, i})$ relative to the fixed population standard deviation $(\sigma_{u, i})$ of 0.2. 
%We reiterate that instead of altering the variance of the entire user population as seen in Section \ref{sec:synthetic:var}, we only change the variance of one user. 
%This allows us to isolate the root cause of a high acceptance region to the properties of a specific user's features.
% \paragraph{Results}
It is clear the overall AR, FRR and FPR of the users is not affected by changing feature variance of a single user, despite the isolated user's samples included as part of training and testing data of other users. Conversely, when viewing the AR, FRR and FPR of the isolated user, we observe a slight increase in FRR and FPR as the relative variance increases. This is due to the positive samples being spread out due to increased variance in the isolated user's samples. However, this is accompanied by a substantially large increase in the acceptance region of this user, approaching 1, i.e., the entire feature space. Furthermore, this trend is visible for all four classifiers.





\subsubsection{Fixed Isolated User Variance and Variable Population Variance}



%\subsubsection{The population's variance with respect to a user's fixed variance.}

In this experiment, we fix the variance $\sigma^2_{u_\text{tgt}, i}$ of the isolated user ($u_\text{tgt}$) at $(0.2)^2$. The $\sigma^2_{u, i}$ of the remaining population is sampled from a normal distribution $\sigma_{u, i} \leftarrow \mathcal{N}(\mu_{i}, \sigma^2_{i})$.
Where $\mu_{i}$ and $\sigma_{i}$ is sampled from the following distributions
$\mathcal{N}(\mu_{\text{mn}}, \sigma^2_{\text{mn}}) = \mathcal{N}(\mu_{\text{mn}}, 0.05^2)$ and $\mathcal{N}(\mu_{\text{var}}, \sigma^2_{\text{var}}) = \mathcal{N}(0.03, 0.02^2)$, respectively. $\mu_{\text{mn}}$ is varied between 0.05 and 0.35 in increments on 0.05
%
%($\mu_{SD} \pm 0.05$) and the SD of the feature SD sampled from ($0.03 \pm 0.02$), where $\mu_{SD}$ is varied between 0.05 and 0.35 in increments on 0.05. 
This sampling permits a small amount of variation between features.

The results are shown in Figure \ref{fig:isolate_otherv}. Inspecting the average AR, FRR and FPR of the system, it is evident there is a continual increase of all 3 metrics as the relative variance increases. This increase is expected as the majority of users' feature values have high variance, presenting an increasingly difficult problem for the machine learner to reduce misclassification errors. However, in all four classifiers the average AR curve is either comparable or lower than the FPR curve as the relative variance increases. For the isolated user, we see that when the relative variance of all other users is lower than this user (to the left), the AR is significantly higher even though the FPR and FRR are minimal in all four classifiers. This shows that less variance in the population samples will result in a high AR, as the classifier need not tighten AR around the true positive region, due to lack of high variance negative samples. On the other hand, AR of the isolated user decreases as the relative variance of the population increases.

% Alluding to the rectangular area first introduced in Section~\ref{sec:attack_def}, user data with higher variance will result in larger feature areas, thus increasing the theoretical ideal AR of a user. We have previously observed the AR to be orders of magnitude larger than the ideal area, we now observe that an relative increase of the ideal area will also increase the resulting AR learned by the model. \ben{This loose correlation may also an indicator for why the touch dataset was observed to have such high ARs, the smaller dimensionality will result in proportionally larger feature rectangles, and hence AR.}. Likewise for the isolated user, when faced with a relatively high fixed variance of the target user (to the left), their feature area, in addition with the acceptance region of the target user will be high.

% \hassan{Need to point out that the FPR and FRR are still reasonable even though AR grows significantly}
% \hassan{Also, need to relate this to points made at the end of Section~\ref{sec:attack_def}}\ben{edit above}

% As such we speculate that a high acceptance region is a result of a relatively higher variance in a user's features in comparison to the remainder of the population. Thus models performing poorly in AR may be victims to the dataset their models are trained on. It may be possible to restrict the acceptance region of a user with relatively higher variance by training their model with data that possesses similar variance characteristics. Or as we observe in the next section with the inclusion of beta noise.

%\red{Possibly also run an Isolated test with the addition of our beta distribution noise as outlined in Section \ref{sec:mitigation}.}



\blue{
\subsection{On Distance Based Classifiers}
\label{sec:distance_classifier}
}

\blue{
As noted earlier, it has been stated that random inputs are ineffective against distance-based classification algorithms~\cite{pagnin2014leakage}. This is in contrast to the machine learning based algorithms evaluated in this paper. 
We take a brief interlude to experimentally evaluate this claim on the cosine similarity distance-based classifier. 
%, is in-fact able to near perfectly reject random inputs, while machine learning based algorithms on an identically configured synthetic dataset does not.
We sample 50 features with means distributed as 
$\mathcal{N}(\mu_{\text{mn}}, \sigma^2_{\text{mn}}) = \mathcal{N}(0.2, 0.05^2)$ and variance distributed as $\mathcal{N}(\mu_{\text{var}}, \sigma^2_{\text{var}}) = \mathcal{N}(0.03, 0.02^2)$. Cosine similarity is computed between two vectors of the same length. As our positive training data contains more than one training sample, we use the average of these samples as the representative template of the user~\cite{chauhan2016gesture}. We use a fixed number of 50 users, with the experiment repeated 50 times. Recall that our evaluation at each threshold is best-effort; we use 1,000 threshold bins for the evaluation of the cosine similarity classifier, since the FRR and FPR rapidly change over a small range of thresholds.

Figure~\ref{fig:cosine_results} displays three classical machine learning algorithms of linear SVM, radial SVM, and random forests, alongside a distance-based cosine similarity classifier. 
%We note that while conventionally the threshold of a distance classifier is set by the negative class during training. However as it was desirable to view the ROC behavior, this conventionally learned threshold serves no purpose. 
It is clear from the figure, that the AR is near zero for cosine similarity, unlike the other classifiers using the same synthetic dataset. This, however, comes at the cost of higher EER. This suggests that distance-based classifiers are effective in minimizing the AR of model, but at the expense of accuracy of the system. We leave further investigation of distance-based classifiers as future work.
%, although in this instance at the cost of a higher EER.

\subsection{Effects of Increasing Synthetic Users}
\label{sec:vary_users}
The real-world datasets used in Section~\ref{sec:realscheme} have a variable number of users. Our binary classification task aggregates negative user samples into a negative class, resulting in distributions and variances of the negative class which depend on the number of users in the datasets. Thus, in this test we investigate the impact on TPR, FPR and AR by varying the number of users in the dataset. We use the synthetic dataset configured in the same manner as in Section~\ref{sec:distance_classifier}. We increase the number of users within the synthetic dataset, from 25 to 150, in increments of 25. Note that the split between positive and negative samples is still balanced (see Remark~\ref{rem:balanced}).

In Figure \ref{fig:vary_users}, we observe that with the addition of more users, there is a slight increase in the FPR. This is expected as the likelihood of user features being similar between any two users will increase with more users in the population. As the training of the classifier uses samples from other users as a negative class, the increased number of negative users slightly lowers the AR of the classifier, with an increased variation of the negative training set (from additional users) covering more of the feature space. However, both these changes are relatively minor despite the multi-fold increase in the number of users. Thus, the AR of the classifiers remains relatively stable with an increasing number of users. 


% In Figure \ref{fig:vary_users}, we observe that with the addition of more users, there is a slight increase in the FPR. This is expected as the likelihood of user features being similar between any two users will increase with more users in the population. As the training of the classifier uses samples from other users as a negative class, the increased number of negative users slightly lowers the AR of the classifier, with an increased variation of the negative training set (from additional users) covering more of the feature space. However, both these changes are relatively minor despite the multi-fold increase in the number of users. Thus, the AR of the classifiers remains relatively stable with an increasing number of users. 
}




%\subsubsection{Varying Number of Users}

%\hassan{Once again AR is higher than FPR. Why would this be related to the birthday problem?} \ben{The birthday problem states that in a room of people, the probability that two users have the same birthday increases exponentially. In the case of the FPR of our authentication system, the probability that another user has a similar biometric profile/sample to our target user also increases exponentially.}


%%%
% \hassan{I am not sure if 50 features per user is common? Can we use a more typical number?}\ben{It would be hard to definitively say what a typical number of features is, as later in the Facial authentication section, each face image has 512 features, and 1024 for Voice authentication.}\ben{It will also be a good idea to use a smaller number of features, to visually show a larger variation in the FPRs and ARs, when we change the number of users.}
%%%



